Towards Long-Range 3D Object Detection for Autonomous Vehicles

3D object detection at long range is crucial for ensuring the safety and efficiency of self driving vehicles, allowing them to accurately perceive and react to objects, obstacles, and potential hazards from a distance. But most current state of the art LiDAR based methods are range limited due to sparsity at long range, which generates a form of domain gap between points closer to and farther away from the ego vehicle. Another related problem is the label imbalance for faraway objects, which inhibits the performance of Deep Neural Networks at long range. To address the above limitations, we investigate two ways to improve long range performance of current LiDAR based 3D detectors. First, we combine two 3D detection networks, referred to as range experts, one specializing at near to mid range objects, and one at long range 3D detection. To train a detector at long range under a scarce label regime, we further weigh the loss according to the labelled point's distance from ego vehicle. Second, we augment LiDAR scans with virtual points generated using Multimodal Virtual Points (MVP), a readily available image-based depth completion algorithm. Our experiments on the long range Argoverse2 (AV2) dataset indicate that MVP is more effective in improving long range performance, while maintaining a straightforward implementation. On the other hand, the range experts offer a computationally efficient and simpler alternative, avoiding dependency on image-based segmentation networks and perfect camera-LiDAR calibration.

==> sections/EXPERIMENTS/comparison_to_baseline.tex <==
% \subsection{Runtime}
\subsection{Comparison to Baseline}     
\label{subsec:comparison_baseline}

\input{tables/Baseline_comparison}

%A detailed 
A comparison between our algorithms and their respective baselines as a function of the range is shown in~\Cref{tab:commparison_baseline}. To guarantee a fair comparison, we re-train the baseline networks for six epochs using \gls{cbgs}, which we denote by $*$. We also provide the performance reported by the authors of the baseline for completeness, denoted by $\dagger$. For \gls{fsd}, we reduce the minimum points for clustering from two to one, to enable clustering at long range. It's observed that using \gls{cbgs} seems to slightly benefit long range performance. For both baselines, a consistent improvement across ranges can be attributed to the respective range experts specializing in their domain. Nevertheless, very little improvement is observed in 200-250\si{m} range, perhaps because labels in this range constitute only 0.3\% of the dataset, as shown in \cref{fig:Statistics_dataset}. Our results underscore the substantial room for improvement within the current state-of-the-art for long-range 3D detection. 
%Our results also demonstrate that there is a large scope for improvement in current state-of-the-art.

%To guarantee a fair comparison, we re-train the baseline network for the same number of epochs with MVP and range weights (our contribution) and without them (fair comparison). In both cases we use CBGS \cite{zhu2019class} while training. We also provide the performance reported by the authors of the baseline for completeness. 


%By increasing the training time, a slight improvement in performance is observed, however, the MVP and range weighting clearly boost the performance. This improvement is observed for most\footnote{In the 0-50~\si{m} range, the additional training epochs with \gls{cbgs} result in a degrade in performance, making the original \gls{fsd}v2$\dagger$ algorithm the most optimal at this range.}  distances, but it is especially beneficial for objects above 50~\si{m} which are traditionally disregarded by most short range algorithms.



==> sections/EXPERIMENTS/effect_2d_backbone.tex <==
% \subsection{Ablation Studies}   \label{subsec:ablation_studies} 
\subsection{Effect of image segmentation}   \label{subsec:2d_backbone} 
%\textbf{Effect of 2D backbone:}
%We analyze the effect of the image segmentation quality on the performance 
% In order to analyze the robustness of the proposed approach to image segmentation, 
To analyze the impact of image segmentation backbone on the performance of our proposed approach, 
we replace HTC~\cite{chen2019hybrid} (default 2D segmentor) with Mask RCNN~\cite{he2017mask},  another well known image segmentor.
%, albeit with a lower mask and box mAP. 
As shown in \Cref{table:effect_2d_backbone}, our finetuned RangeFSD with Mask RCNN gives similar results to HTC, demonstrating robustness to the 2D segmentor employed. On the other hand, the significantly higher mask and box mAP for HTC indicates that while both the segmentors seem to detect mid range objects equally well, HTC could be better at detecting small objects.
%, including those at long range. 
%Some of these could well be at long range and out of reach for current \gls{lidar}s, in which case a \gls{lidar}-only detector cannot detect them.
Some of these small objects could very well be at large distances, outside the reach of \gls{lidar} points, making it impossible for a \gls{lidar}-only detector to detect them.
\input{tables/Ablation_img_backbone}



==> sections/EXPERIMENTS/performance_breakdown.tex <==
\subsection{Performance Breakdown}  \label{subsec:performance_breakdown}
Our contribution can be divided into two components: implementation of \gls{mvp} and range experts. In order to assess the impact of each component on our final state-of-the art algorithms, a detailed performance breakdown, shown in \Cref{tab:perf_breakdown}, is performed. 

\input{tables/Performance_breakdown}

The impact of \gls{mvp}
% with and without finetuning 
is studied independently for the \gls{fsd} and RangeFSD. 
% The finetuning of \gls{mvp} proves to be crucial in both cases, where a drop in performance is observed when implementing the \gls{mvp} without finetuning.
It was observed that finetuning after adding virtual points is crucial for both the cases. A significant drop in performance is observed when applying \gls{mvp} without finetuning.
This drop could be explained by a shift in point distribution caused by \gls{mvp}. The \gls{lidar} pre-segmentor, used by both baselines, is negatively affected by this shift and hence needs to be finetuned. Overall, \gls{mvp} contributes to about 1.7\% increase in \gls{map}, whereas the range expert contributes about 0.4\% \gls{map}. Although a higher boost in performance arises from \gls{mvp}, a combination of \gls{mvp} and range experts is required to maximise the performance of \gls{fsd}. 

% The impact of MVP with and without finetuning is studied independently for the FSD and RangeFSD algorithms. The finetuning of MVP proves to be crucial in both cases, where a drop in performance is observed when implementing the MVP without finetuning. This drop can be attributed to a shift in point distribution caused by MVP.  
%The finetuned MVP implementation drastically improves the performance for both algorithms at all distances. Furthermore, for all tested configurations, RangeFSD performs better or than FSD for distances below 200 m. No improvement is observed for objects above 200 m. %Depending on the distance, the boost in performance arising from the range experts is between 0--40\% lower when combined with MVP than when applied alone. This indicates that, 
%The overall best performance is obtained when combining both MVP with finetuning and range experts. It is worth noting that, for distances below 150 m, the boost in performance from the range experts is up to 40\% lower when combined with MVP than when applied alone. This indicates a small correlation between the correctly classified objects between MVP and range experts at this distances. No correlation is observed for distances above 150 m. A higher boost in performance arises from implementing MVP, however, the combination of MVP and range experts is required to maximise the performance of the FSD algorithm.


==> sections/EXPERIMENTS/strategy_for_training_long_range.tex <==
\subsection{Strategies for Training Long Range Detector}   \label{subsec:range_thresh_and_wt}

\input{tables/Ablation_range_thresholding}

The effect of range threshold and range weighing on the \gls{fsd} trained using \gls{mvp} is summarised in~\Cref{tab:range_ablation}. The general experts are optimised to target objects in the full 0-250~\si{m} range while the long- (mid-) range experts aim to maximise the performance for distances $>$ ($\leq$) 100~\si{m}. 
~\Cref{table:range_wts} further denotes the range weights for both mid and long range experts for different values of range thresholding $r_1$ and $r_2$. These weights are computed using \cref{eq:weights} together with the the bin-wise label statistics of the training set, which were shown in \cref{fig:Statistics_dataset}.


%Given the large difference in the number of labeled objects as a function of their distance, which was illustrated in \cref{fig:Statistics_dataset}, it is only natural that the FSD$_{0-250}$ algorithm, which is used as baseline in this experiment, performs best for near objects within distances below 50 m. In order to improve performance on long range points, two different approaches are tested: range thresholding and range weighing. The former consists on training the algorithm using only a subset of objects with a specific distance we are aiming to target. The latter consists on reducing the imbalance of labeled objects between distances by increasing the impact on the loss function on objects that are further away. 


\input{tables/Method_range_weighing_values}

The range weights, which are implemented in FSD$_{0-250}^{w}$, show a performance improvement in the 50-150~\si{m} range with respect to FSD$_{0-250}$ and a performance degrading in the below 50~\si{m} range. We also train long-range experts using range thresholding of $50-250$~\si{m} and $100-250$~\si{m} with and without range weights for comparison. In particular, FSD$_{100-250}$ corresponds to simply finetuning the network for long-range points, and it performs the worst in 100-150~\si{m} range. It is observed that range weighing leads to slight improvements for both long-range experts. Moreover, it is found that the best performance for a range bin $b$ can be obtained by using range thresholding from bin $b-1$ in combination with range weighing i.e. the best performance at $100-150$~\si{m} is obtained by FSD$_{50-250}^{w}$. We also train a short range expert, referred as FSD$_{0-100}$, using range thresholding of $0-100$~\si{m}. Range weights are not applied in this case in order not to degrade the performance at $0-50$~\si{m}. As expected, the short range expert results in the most optimal performance for objects at $0-50$~\si{m}, while the performance at  $50-100$~\si{m} is only degraded by 0.1\% with respect to FSD$_{0-250}^{w}$. Based on the results, we choose FSD$_{0-100}$ and FSD$_{50-250}^{w}$ as the mid- and long- range experts, and merge them to form RangeFSD, a network with high performance at both mid and long range.


%The range weights, which are implemented in FSD$_{0-250}^{w}$, show a performance improvement in the range 50-150 range with respect to FSD$_{0-250}$ and a performance degrading in the below 50 m range. Long range experts are trained using range thresholding of $50-250$ and $100-250$ with and without range weights in order to improve the performance of objects at long range. The best performance for far away objects in the $100-200$ range is found when combining both approaches. In particular, it is found that the best performance for a range bin $n$ can be obtained by using range thresholding from bin $n-1$ in combination with range weighing i.e. the best performance at $100-150$ is obtained by FSD$_{50-250}^{w}$, while the best performance at  $150-200$  is obtained by FSD$_{100-250}^{w}$. A short range expert, referred as FSD$_{0-100}$, is also trained using range thresholding of $0-100$. Range weights are not applied in this case in order to not degrade the performance at $0-50$ m. As expected, the short range expert results in the most optimal performance for objects at $0-50$ m, while the performance at  $50-100$ m is only degraded by 0.1 with respect to FSD$_{0-250}^{w}$, which yields the best performance for that range. The mid- and long- range experts, FSD$_{0-100}$ and FSD$_{50-250}^{w}$, are merged to form RangeFSD, a network with high performance at both mid and long range.


==> tables/Ablation_range_merging.tex <==
\begin{table}[h] 
\centering 
\scriptsize
\caption{Comparison of RangeFSD and its components, the best-performing mid and long range experts.} 
\label{tab:range_ablation}
\renewcommand{\arraystretch}{1.2}
% \setlength{\tabcolsep}{3pt}\begin{tabular}{l|c|c|c|c|c|c|c} 
 \setlength{\tabcolsep}{2.5pt}\begin{tabular}{l|l|c|c|ccccc}
 \hline 
\multirow{2}{*}{} & \multirow{2}{*}{} & Range & \multirow{2}{*}{} & \multirow{2}{*}{} & \multirow{2}{*}{} & \multirow{2}{*}{} & \multirow{2}{*}{} & \multirow{2}{*}{} \\
Expert &  Method  &  Weights & 0-250 & 0-50 & 50-100 & 100-150 & 150-200 & 200-250 \\
 \hline
  Mid & FSD$_{0-100}$ &  $\times$  & 31.3 & 46.9 & 16.9 & 0.5 & - & -\\  \hline 
 Long & FSD$_{50-250}^w$ & \checkmark & 6.0 & 0.3 & 16.5 & 6.1 & 2.0 & 0.5\\ \cline{2-9}
 General & FSD$\_$Range$^{*}$ & \checkmark  & 31.9 & 46.9 & 16.9 & 5.8 & 2.0 & 0.5  \\  \hline

\end{tabular} 
\end{table} 


==> tables/Ablation_range_thresholding.tex <==
\begin{table}[h] 
\centering 
\scriptsize
\caption{Effect of Range thresholding and range weighing on mAP.} 
\label{tab:range_ablation}
\renewcommand{\arraystretch}{1.2}
% \setlength{\tabcolsep}{3pt}\begin{tabular}{l|c|c|c|c|c|c|c} 
 \setlength{\tabcolsep}{2pt}\begin{tabular}{l|l|c|c|ccccc}
 \hline 
\multirow{2}{*}{} & \multirow{2}{*}{} & Range & \multirow{2}{*}{} & \multirow{2}{*}{} & \multirow{2}{*}{} & \multirow{2}{*}{} & \multirow{2}{*}{} & \multirow{2}{*}{} \\
Expert &  Method  &  Weights & 0-250 & 0-50 & 50-100 & 100-150 & 150-200 & 200-250 \\
%\r'ot{Expert} &  \rot{Method}  &  \rot{Weights} & \rot{0-250} & \rot{0-50} & \rot{50-100} & \rot{100-150} & \rot{150-200} & \rot{200-250} \\
 \hline
  \multirow{2}{*}{General} & FSD$_{0-250}$ & $-$ & 31.5 & 46.4 & 16.6 & 5.4 & 1.8 & 0.5\\ 
 & FSD$_{0-250}^w$ & \checkmark & 31.3 & 45.9 & 17.0 & 5.7 & 1.8 & 0.4\\ \hline
%& \textcolor{blue}{RangeFSD}$^{*}$ & \checkmark  & 31.9 & 46.9 & 16.9 & 5.8 & 2.0 & 0.5  \\ \hline

   Mid & FSD$_{0-100}$ *&  $-$  & - & 46.9 & 16.9 & 0.5 & - & -\\ % \hline 
 \multirow{1}{*}{Long} & FSD$_{50-250}$ * & $-$ & - & - & 16.6 & 5.9 & 2.0 & 0.6\\
 %& FSD$_{50-250}^w$ *& \checkmark & 6.0 & - & 16.5 & 6.1 & 2.0 & 0.5\\ \cline{2-9}
 %& FSD$_{100-250}$ & $-$ & 1.0 & - & - & 4.9 & 2.0 & 0.6\\
 %& FSD$_{100-250}^w$ & \checkmark & 1.1 & - & - & 5.0 & 2.1 & 0.5\\ 
 \hline
 Merged & $RangeFSD^{*}$ & $-$  & 31.9 & 46.9 & 16.9 & 5.8 & 2.0 & 0.5  \\  \hline

\end{tabular} 
\end{table} 


% \setlength{\tabcolsep}{3pt}\begin{tabular}{l|c|c|c|c|c|c|c} 
%  % \setlength{\tabcolsep}{2pt}\begin{tabular}{l|cccccccc}
%  \hline 
%   Method  & Range Weighting & 0-250 & 0-50 & 50-100 & 100-150 & 150-200 & 200-250 \\
%  \hline
%  FSD$_{0-100}$ &  & 0 & 0 & 0 & 0 & 0 & 0\\ \hline
%  \multirow{1}{*}{FSD$_{0-250}$} & & 0 & 0 & 0 & 0 & 0 & 0\\ 
%  \multirow{1}{*}{FSD$_{0-250}^w$} & \checkmark & 0 & 0 & 0 & 0 & 0 & 0\\ \hline
%  \multirow{2}{*}{FSD$_{50-250}$} & & 0 & 0 & 0 & 0 & 0 & 0\\
%  FSD$_{50-250}$ & \checkmark & 0 & 0 & 0 & 0 & 0 & 0\\ \hline
%  \multirow{2}{*}{FSD$_{100-250}$} & & 0 & 0 & 0 & 0 & 0 & 0\\
%  FSD$_{100-250}^w$ & \checkmark & 0 & 0 & 0 & 0 & 0 & 0\\ 
%  \hline 
% \end{tabular} 
% \end{table*} 

==> tables/Baseline_comparison.tex <==
\begin{table}[h] 
\centering 
\scriptsize
% \footnotesize 
\caption{mAP comparison to Baseline. $\dagger$: provided by authors~\cite{fan2022fully}\cite{fan2023fsdv2}. *: re-trained by us.} 
\label{tab:commparison_baseline}
\renewcommand{\arraystretch}{1.2}
% \setlength{\tabcolsep}{3pt}\begin{tabular}{l|c|c|c|c|c|c|c} 
 \setlength{\tabcolsep}{3pt}\begin{tabular}{l|c|ccccc}
 \hline 
  Method & 0-250 & 0-50 & 50-100 & 100-150 & 150-200 & 200-250  \\
 \hline
 FSD$\dagger$ &  28.5 & 43.7 & 12.6 & 3.3 & 1.0 & 0.3 \\
 FSD* &  29.8 & 44.9 & 14.3 & 4.1 & 1.0 & 0.3 \\ 
 RangeFSD & 31.9 & 46.9 & 16.9 & 5.8 & 2.0 & 0.5 \\ \hline
 FSDv2$\dagger$ & 37.5 & 52.8 & 22.3 & 7.5 & 2.5 & 0.4\\
 FSDv2* & 37.5 & 52.2 & 23.0 & 8.6 & 2.5 & 0.5 \\ 
 RangeFSDv2 & 38.3 & 52.3 & 25.2 & 9.8 & 3.1 & 0.6 \\
 \hline 
\end{tabular} 
\end{table} 

% \begin{table}[htbp!] 
% \centering 
% \scriptsize
% % \footnotesize 
% \caption{Comparison to Baseline. $\dagger$: provided by authors~\cite{fan2022fully}\cite{fan2023fsdv2}. *: re-trained by us.} 
% \label{tab:commparison_baseline}
% \renewcommand{\arraystretch}{1.2}
% % \setlength{\tabcolsep}{3pt}\begin{tabular}{l|c|c|c|c|c|c|c} 
%  \setlength{\tabcolsep}{3pt}\begin{tabular}{l|c|ccccc|c}
%  \hline 
%   \multirow{2}{*}{} & \multirow{2}{*}{} & \multirow{2}{*}{} & \multirow{2}{*}{} & \multirow{2}{*}{} & \multirow{2}{*}{} & \multirow{2}{*}{} & Runtime \\
%   Method & 0-250 & 0-50 & 50-100 & 100-150 & 150-200 & 200-250 & (msec) \\
%  \hline
%  FSD$\dagger$ &  28.5 & 43.7 & 12.6 & 3.3 & 1.0 & 0.3 & \\
%  FSD* &  29.8 & 44.9 & 14.3 & 4.1 & 1.0 & 0.3 & \\ 
%  RangeFSD & 31.9 & 46.9 & 16.9 & 5.8 & 2.0 & 0.5 & \\ \hline
%  FSDv2$\dagger$ & 37.5 & 52.8 & 22.3 & 7.5 & 2.5 & 0.4 &\\
%  FSDv2* & 37.5 & 52.2 & 23.0 & 8.6 & 2.5 & 0.5 &\\ 
%  RangeFSDv2 & 38.3 & 52.3 & 25.2 & 9.8 & 3.1 & 0.6 & \\
%  \hline 
% \end{tabular} 
% \end{table} 


==> tables/Custom_Table.tex <==
\begin{table*}[t] 
\centering 
\footnotesize 
\caption{The AP (AR) are reported for the different classes, methods and ranges.} 
 
\begin{tabular}{ll|ccccccccccccccccccccccccccc} 
 
 \hline 
 Range & Method  & \rot{Articulated Bus } & \rot{Bicycle } & \rot{Bicyclist } & \rot{Bollard } & \rot{Box Truck } & \rot{Bus } & \rot{Constr. Barrel } & \rot{Const. Cone } & \rot{Dog } & \rot{Large Vehicle } & \rot{Message Board Trailer } & \rot{M. Ped. Cross. Sign } & \rot{Motorcyle } & \rot{Motorcyclist } & \rot{Pedestrian } & \rot{Vehicle } & \rot{School Bus } & \rot{Sign } & \rot{Stop Sign } & \rot{Stroller } & \rot{Truck } & \rot{Truck Cab } & \rot{Trailer } & \rot{Wheelchair } & \rot{Wheeled Device } & \rot{Wheeled Rider } & \rot{Average All Classes }\\ 
\hline 
\multirow{3}{*}{0-250 m}& Default & $19.3$ ($31.9$)& $37.9$ ($49.6$)& $34.1$ ($48.5$)& $46.9$ ($59.2$)& $37.7$ ($47.3$)& $40.8$ ($49.1$)& $44.4$ ($50.9$)& $43.7$ ($53.4$)& $10.2$ ($28.4$)& $5.8$ ($20.2$)& $0.0$ ($0.0$)& $26.5$ ($43.0$)& $48.2$ ($60.1$)& $39.9$ ($63.2$)& $63.9$ ($70.6$)& $70.5$ ($74.3$)& $29.5$ ($36.7$)& $11.5$ ($30.1$)& $28.9$ ($40.5$)& $12.8$ ($41.2$)& $20.7$ ($42.1$)& $12.0$ ($20.3$)& $25.6$ ($33.1$)& $7.1$ ($19.4$)& $14.2$ ($28.7$)& $9.0$ ($23.5$)& $28.5$ ($41.0$) \\ 
 & IMFSD & $19.1$ ($32.8$)& $37.6$ ($50.0$)& $32.5$ ($48.7$)& $46.9$ ($59.2$)& $35.9$ ($47.4$)& $39.4$ ($49.8$)& $43.9$ ($51.2$)& $43.5$ ($53.7$)& $10.3$ ($29.2$)& $5.2$ ($20.8$)& $0.0$ ($0.0$)& $25.3$ ($43.4$)& $48.4$ ($60.9$)& $38.9$ ($63.6$)& $62.7$ ($70.6$)& $69.6$ ($74.6$)& $29.0$ ($38.2$)& $10.6$ ($30.3$)& $28.6$ ($40.4$)& $12.8$ ($41.2$)& $20.3$ ($44.6$)& $17.7$ ($28.6$)& $24.7$ ($33.9$)& $6.6$ ($20.4$)& $14.2$ ($28.9$)& $8.7$ ($23.8$)& $28.2$ ($41.8$) \\ 
 & Default+MVP & $17.2$ ($27.7$)& $38.7$ ($50.7$)& $35.2$ ($49.8$)& $49.4$ ($60.5$)& $37.6$ ($47.3$)& $40.8$ ($49.6$)& $48.6$ ($55.1$)& $44.3$ ($54.0$)& $2.4$ ($28.9$)& $5.3$ ($21.8$)& $0.0$ ($9.9$)& $25.1$ ($40.7$)& $49.2$ ($60.6$)& $36.9$ ($62.6$)& $66.0$ ($72.3$)& $72.5$ ($76.4$)& $28.6$ ($35.7$)& $10.7$ ($29.8$)& $29.2$ ($40.8$)& $9.1$ ($41.6$)& $21.0$ ($43.2$)& $17.6$ ($26.4$)& $26.9$ ($34.0$)& $0.9$ ($19.2$)& $15.0$ ($29.7$)& $8.1$ ($22.3$)& $28.3$ ($41.9$) \\ 
 \hline 
 \multirow{3}{*}{50 m}& Default & $33.5$ ($47.0$)& $50.0$ ($63.8$)& $59.8$ ($73.6$)& $62.3$ ($73.9$)& $65.5$ ($75.0$)& $69.0$ ($75.8$)& $73.7$ ($79.6$)& $58.0$ ($68.3$)& $12.1$ ($34.0$)& $11.6$ ($37.7$)& $0.0$ ($0.0$)& $54.2$ ($73.6$)& $63.6$ ($75.4$)& $63.4$ ($84.0$)& $81.0$ ($85.5$)& $88.9$ ($91.3$)& $72.2$ ($79.0$)& $19.8$ ($46.5$)& $50.1$ ($64.7$)& $16.9$ ($53.7$)& $29.4$ ($54.1$)& $17.5$ ($25.6$)& $40.5$ ($50.0$)& $9.9$ ($27.8$)& $19.4$ ($38.3$)& $14.1$ ($33.2$)& $43.7$ ($58.1$) \\ 
 & IMFSD & $33.9$ ($48.8$)& $49.7$ ($64.1$)& $57.1$ ($74.1$)& $62.3$ ($73.9$)& $64.4$ ($75.1$)& $67.6$ ($76.2$)& $72.8$ ($79.9$)& $57.7$ ($68.7$)& $12.3$ ($34.8$)& $10.4$ ($39.0$)& $0.0$ ($0.0$)& $54.6$ ($75.8$)& $63.8$ ($76.4$)& $61.5$ ($84.2$)& $80.0$ ($85.5$)& $88.9$ ($91.3$)& $71.0$ ($80.2$)& $19.7$ ($46.7$)& $50.1$ ($64.7$)& $16.9$ ($53.5$)& $28.9$ ($56.8$)& $27.4$ ($38.8$)& $39.4$ ($50.7$)& $9.2$ ($29.1$)& $19.4$ ($38.6$)& $13.4$ ($33.4$)& $43.6$ ($59.2$) \\ 
 & Default+MVP & $29.7$ ($40.7$)& $50.8$ ($64.6$)& $61.4$ ($74.7$)& $63.9$ ($74.2$)& $64.8$ ($74.2$)& $67.5$ ($74.6$)& $75.7$ ($80.7$)& $58.4$ ($68.3$)& $2.9$ ($34.3$)& $10.3$ ($36.7$)& $0.0$ ($0.0$)& $51.3$ ($70.7$)& $64.3$ ($75.5$)& $59.8$ ($81.0$)& $81.7$ ($85.8$)& $89.0$ ($91.4$)& $70.4$ ($78.5$)& $18.6$ ($45.9$)& $50.5$ ($65.2$)& $12.7$ ($54.9$)& $29.9$ ($55.6$)& $29.4$ ($37.2$)& $42.6$ ($51.1$)& $1.4$ ($27.1$)& $20.8$ ($39.3$)& $13.6$ ($31.4$)& $43.1$ ($58.2$) \\ 
 \hline 
 \multirow{3}{*}{100 m}& Default & $5.7$ ($20.2$)& $9.2$ ($21.8$)& $19.7$ ($44.5$)& $16.3$ ($36.6$)& $23.7$ ($38.5$)& $30.6$ ($45.2$)& $19.4$ ($32.7$)& $7.0$ ($22.1$)& $2.7$ ($7.0$)& $5.3$ ($21.8$)& $0.0$ ($0.0$)& $10.6$ ($22.5$)& $9.8$ ($33.6$)& $8.0$ ($57.2$)& $40.9$ ($57.3$)& $59.7$ ($67.2$)& $9.4$ ($23.9$)& $4.0$ ($22.8$)& $3.5$ ($17.5$)& $0.0$ ($1.6$)& $18.1$ ($42.6$)& $10.0$ ($20.5$)& $12.1$ ($21.5$)& $1.5$ ($2.0$)& $0.4$ ($4.0$)& $1.5$ ($12.4$)& $12.6$ ($26.8$) \\ 
 & IMFSD & $5.2$ ($21.4$)& $9.1$ ($22.1$)& $18.8$ ($44.7$)& $16.2$ ($36.6$)& $21.7$ ($38.4$)& $29.8$ ($46.3$)& $18.8$ ($33.0$)& $6.7$ ($22.1$)& $3.0$ ($7.2$)& $5.1$ ($22.6$)& $0.0$ ($0.0$)& $10.5$ ($22.8$)& $10.0$ ($34.7$)& $7.7$ ($58.2$)& $40.2$ ($57.4$)& $59.5$ ($67.3$)& $9.2$ ($26.5$)& $4.0$ ($23.1$)& $3.4$ ($17.6$)& $0.0$ ($1.6$)& $18.1$ ($46.6$)& $11.9$ ($24.8$)& $12.4$ ($23.8$)& $1.7$ ($2.0$)& $0.4$ ($4.1$)& $1.5$ ($12.9$)& $12.5$ ($27.6$) \\ 
 & Default+MVP & $6.2$ ($18.5$)& $9.9$ ($22.7$)& $20.5$ ($44.8$)& $21.0$ ($40.2$)& $23.5$ ($37.6$)& $31.1$ ($45.5$)& $26.6$ ($38.7$)& $7.5$ ($23.2$)& $0.6$ ($11.5$)& $5.1$ ($21.7$)& $0.1$ ($10.5$)& $9.4$ ($20.9$)& $9.7$ ($31.5$)& $7.7$ ($55.5$)& $44.0$ ($59.0$)& $60.5$ ($67.7$)& $9.7$ ($22.1$)& $3.4$ ($22.8$)& $3.3$ ($18.1$)& $0.0$ ($1.7$)& $18.6$ ($42.6$)& $8.0$ ($19.1$)& $11.7$ ($21.5$)& $0.1$ ($6.0$)& $0.3$ ($5.6$)& $1.4$ ($8.9$)& $13.1$ ($27.6$) \\ 
 \hline 
 \multirow{3}{*}{150 m}& Default & $4.5$ ($20.0$)& $0.4$ ($3.7$)& $1.5$ ($9.2$)& $1.9$ ($7.4$)& $8.4$ ($22.8$)& $15.3$ ($28.1$)& $1.0$ ($5.7$)& $0.1$ ($0.3$)& $0.0$ ($0.0$)& $1.2$ ($12.2$)& $0.0$ ($0.0$)& $0.1$ ($18.0$)& $0.1$ ($3.9$)& $0.2$ ($6.8$)& $11.2$ ($25.3$)& $26.8$ ($40.4$)& $0.3$ ($6.8$)& $0.4$ ($9.7$)& $0.4$ ($7.6$)& $0.0$ ($0.0$)& $4.7$ ($20.6$)& $2.5$ ($9.3$)& $4.5$ ($8.9$)& $0.0$ ($0.0$)& $0.5$ ($0.7$)& $0.0$ ($0.6$)& $3.3$ ($10.3$) \\ 
 & IMFSD & $3.6$ ($20.1$)& $0.4$ ($3.7$)& $1.5$ ($9.5$)& $1.5$ ($7.4$)& $7.3$ ($23.3$)& $12.0$ ($29.4$)& $1.8$ ($5.8$)& $0.1$ ($0.3$)& $0.0$ ($0.0$)& $1.2$ ($12.4$)& $0.0$ ($0.0$)& $0.1$ ($19.3$)& $0.1$ ($3.9$)& $0.2$ ($6.8$)& $8.1$ ($25.7$)& $22.5$ ($42.0$)& $0.8$ ($8.0$)& $0.4$ ($12.2$)& $0.3$ ($8.6$)& $0.0$ ($0.0$)& $4.6$ ($22.4$)& $4.4$ ($13.1$)& $2.7$ ($9.2$)& $0.0$ ($0.0$)& $0.4$ ($0.7$)& $0.0$ ($0.6$)& $2.8$ ($10.9$) \\ 
 & Default+MVP & $2.2$ ($12.2$)& $1.3$ ($8.2$)& $1.0$ ($12.8$)& $2.9$ ($11.0$)& $9.4$ ($23.5$)& $16.7$ ($30.8$)& $6.3$ ($17.8$)& $2.6$ ($7.1$)& $0.0$ ($0.0$)& $2.4$ ($18.2$)& $0.0$ ($0.0$)& $0.1$ ($12.3$)& $2.2$ ($11.0$)& $1.2$ ($14.0$)& $18.6$ ($36.9$)& $37.4$ ($51.3$)& $0.2$ ($5.9$)& $0.3$ ($8.4$)& $0.2$ ($4.6$)& $0.0$ ($4.2$)& $3.6$ ($25.4$)& $1.6$ ($10.8$)& $3.2$ ($8.1$)& $0.0$ ($0.0$)& $0.0$ ($0.3$)& $0.0$ ($0.6$)& $4.4$ ($12.9$) \\ 
 \hline 
 \multirow{3}{*}{200 m}& Default & $0.2$ ($14.1$)& $0.0$ ($0.0$)& $0.2$ ($0.9$)& $0.0$ ($0.0$)& $3.3$ ($12.6$)& $0.9$ ($7.6$)& $0.1$ ($0.0$)& $0.0$ ($0.0$)& $0.0$ ($0.0$)& $2.3$ ($9.6$)& $0.0$ ($0.0$)& $0.0$ ($0.0$)& $0.0$ ($0.0$)& $0.0$ ($0.0$)& $1.1$ ($3.2$)& $12.1$ ($25.6$)& $0.1$ ($2.9$)& $1.1$ ($3.8$)& $0.1$ ($3.5$)& $0.0$ ($0.0$)& $0.8$ ($6.8$)& $3.7$ ($8.9$)& $0.2$ ($2.0$)& $0.0$ ($0.0$)& $0.0$ ($0.0$)& $0.0$ ($0.0$)& $1.0$ ($3.9$) \\ 
 & IMFSD & $0.2$ ($14.1$)& $0.0$ ($0.0$)& $0.1$ ($0.9$)& $2.2$ ($3.7$)& $1.8$ ($13.6$)& $1.1$ ($8.7$)& $0.5$ ($0.1$)& $0.0$ ($0.0$)& $0.0$ ($0.0$)& $2.3$ ($10.5$)& $0.0$ ($0.0$)& $0.0$ ($0.0$)& $0.0$ ($0.0$)& $0.0$ ($0.0$)& $1.2$ ($7.1$)& $9.6$ ($32.6$)& $0.1$ ($3.0$)& $0.1$ ($4.0$)& $0.1$ ($6.0$)& $0.0$ ($0.0$)& $1.0$ ($8.4$)& $3.7$ ($11.0$)& $0.2$ ($2.5$)& $0.0$ ($0.0$)& $0.0$ ($0.0$)& $0.0$ ($0.0$)& $0.9$ ($4.9$) \\ 
 & Default+MVP & $0.0$ ($3.9$)& $0.0$ ($0.5$)& $0.1$ ($1.3$)& $0.5$ ($0.3$)& $4.6$ ($16.1$)& $3.3$ ($13.5$)& $2.2$ ($4.1$)& $0.0$ ($0.0$)& $0.0$ ($0.0$)& $3.8$ ($16.5$)& $0.0$ ($0.0$)& $0.0$ ($0.0$)& $0.0$ ($0.0$)& $0.0$ ($0.0$)& $4.9$ ($14.6$)& $22.1$ ($39.1$)& $0.0$ ($1.2$)& $0.3$ ($3.9$)& $0.1$ ($2.7$)& $0.0$ ($0.0$)& $0.6$ ($10.3$)& $1.4$ ($11.3$)& $0.7$ ($5.5$)& $0.0$ ($0.0$)& $0.0$ ($0.0$)& $0.0$ ($0.0$)& $1.7$ ($5.6$) \\ 
 \hline 
 \multirow{3}{*}{250 m}& Default & $0.0$ ($0.0$)& $0.0$ ($0.0$)& $0.0$ ($0.0$)& $0.0$ ($0.0$)& $1.3$ ($2.7$)& $0.0$ ($0.0$)& $0.0$ ($0.0$)& $0.0$ ($0.0$)& $0.0$ ($0.0$)& $0.6$ ($2.7$)& $0.0$ ($0.0$)& $0.0$ ($0.0$)& $0.0$ ($0.0$)& $0.0$ ($0.0$)& $0.0$ ($0.0$)& $2.7$ ($7.6$)& $0.0$ ($0.0$)& $0.0$ ($0.0$)& $0.0$ ($0.0$)& $0.0$ ($0.0$)& $2.7$ ($3.2$)& $1.3$ ($4.7$)& $0.0$ ($0.0$)& $0.0$ ($0.0$)& $0.0$ ($0.0$)& $0.0$ ($0.0$)& $0.3$ ($0.8$) \\ 
 & IMFSD & $0.0$ ($0.0$)& $0.0$ ($0.0$)& $0.0$ ($0.0$)& $0.0$ ($0.0$)& $0.9$ ($2.6$)& $0.0$ ($0.8$)& $0.0$ ($0.0$)& $0.0$ ($0.0$)& $0.0$ ($0.0$)& $0.4$ ($2.8$)& $0.0$ ($0.0$)& $0.0$ ($0.0$)& $0.0$ ($0.0$)& $0.0$ ($0.0$)& $0.1$ ($0.3$)& $2.8$ ($15.0$)& $0.0$ ($0.0$)& $0.0$ ($0.5$)& $0.3$ ($5.3$)& $0.0$ ($0.0$)& $2.7$ ($3.2$)& $1.3$ ($4.7$)& $0.0$ ($0.0$)& $0.0$ ($0.0$)& $0.0$ ($0.0$)& $0.0$ ($0.0$)& $0.3$ ($1.3$) \\ 
 & Default+MVP & $0.0$ ($0.0$)& $0.0$ ($0.0$)& $0.0$ ($0.0$)& $0.0$ ($0.0$)& $3.6$ ($6.0$)& $0.1$ ($1.9$)& $0.0$ ($0.0$)& $0.0$ ($0.0$)& $0.0$ ($0.0$)& $1.5$ ($4.8$)& $0.0$ ($0.0$)& $0.0$ ($0.0$)& $0.0$ ($0.0$)& $0.0$ ($0.0$)& $0.0$ ($0.0$)& $6.5$ ($15.7$)& $0.0$ ($0.0$)& $1.0$ ($2.0$)& $0.0$ ($0.0$)& $0.0$ ($0.0$)& $0.3$ ($4.5$)& $1.5$ ($7.1$)& $0.4$ ($0.4$)& $0.0$ ($0.0$)& $0.0$ ($0.0$)& $0.0$ ($0.0$)& $0.6$ ($1.6$) \\ 
 \hline 
 \hline 
\end{tabular} 
\end{table*} 


==> tables/Custom_Table_AP+AR.tex <==
\begin{table*}[t] 
\centering 
\footnotesize 
\caption{The AP are reported for the different classes, methods and ranges.} 
 
\setlength{\tabcolsep}{2pt}\begin{tabular}{ll|cccccccc} 
 
 \hline 
 Range & Method  & \rot{Vehicle } & \rot{Pedestrian } & \rot{Const. Cone } & \rot{Constr. Barrel } & \rot{Bollard } & \rot{Box Truck } & \rot{Large Vehicle } & \rot{Average All Classes }\\ 
\hline 
\multirow{4}{*}{0-250 m}& FSD (6 epochs) & $71.5$ ($75.4$)& $66.4$ ($72.2$)& $45.6$ ($54.9$)& $52.7$ ($58.8$)& $51.5$ ($61.4$)& $37.3$ ($46.6$)& $5.6$ ($19.4$)& $29.8$ ($42.1$) \\ 
 & FSD+MVP Long (0-250m with range weights, 3 epochs)  & $74.3$ ($78.1$)& $68.7$ ($74.7$)& $54.2$ ($63.1$)& $57.8$ ($63.8$)& $51.9$ ($62.3$)& $38.7$ ($48.8$)& $5.6$ ($22.6$)& $31.3$ ($43.9$) \\ 
 & FSD+MVP Short (<100 m, 3 epochs) & $68.1$ ($70.7$)& $67.0$ ($71.8$)& $54.5$ ($62.3$)& $56.2$ ($60.3$)& $53.0$ ($61.9$)& $37.0$ ($44.9$)& $5.6$ ($17.9$)& $31.2$ ($41.7$) \\ 
 & FSD+MVP (3 epochs) & $74.5$ ($78.3$)& $69.1$ ($74.8$)& $53.2$ ($62.0$)& $57.5$ ($63.5$)& $52.3$ ($62.1$)& $38.0$ ($47.7$)& $5.7$ ($20.9$)& $31.5$ ($43.4$) \\ 
 \hline 
 \multirow{4}{*}{50 m}& FSD (6 epochs) & $89.0$ ($91.3$)& $82.0$ ($86.0$)& $59.6$ ($68.9$)& $79.6$ ($83.8$)& $66.0$ ($75.0$)& $64.2$ ($72.9$)& $10.7$ ($35.1$)& $44.9$ ($59.3$) \\ 
 & FSD+MVP Long (0-250m with range weights, 3 epochs)  & $88.9$ ($91.4$)& $82.5$ ($86.5$)& $68.1$ ($76.2$)& $82.9$ ($86.4$)& $65.2$ ($74.6$)& $63.9$ ($73.1$)& $10.0$ ($37.1$)& $45.9$ ($59.9$) \\ 
 & FSD+MVP Short (<100 m, 3 epochs) & $89.2$ ($91.6$)& $82.9$ ($86.8$)& $68.6$ ($75.8$)& $83.4$ ($86.6$)& $67.0$ ($75.4$)& $65.3$ ($74.1$)& $11.2$ ($36.6$)& $46.9$ ($59.5$) \\ 
 & FSD+MVP (3 epochs) & $89.0$ ($91.5$)& $82.9$ ($86.7$)& $67.1$ ($75.2$)& $82.3$ ($85.7$)& $65.8$ ($74.7$)& $64.5$ ($73.5$)& $9.8$ ($34.7$)& $46.4$ ($59.4$) \\ 
 \hline 
 \multirow{4}{*}{100 m}& FSD (6 epochs) & $61.7$ ($69.1$)& $46.0$ ($60.8$)& $9.6$ ($26.5$)& $32.4$ ($44.2$)& $23.5$ ($41.2$)& $24.0$ ($39.0$)& $5.9$ ($20.2$)& $14.3$ ($28.2$) \\ 
 & FSD+MVP Long (0-250m with range weights, 3 epochs)  & $65.8$ ($72.5$)& $52.8$ ($66.1$)& $20.6$ ($38.7$)& $41.6$ ($53.3$)& $28.3$ ($44.7$)& $27.2$ ($42.3$)& $7.3$ ($25.6$)& $17.0$ ($31.5$) \\ 
 & FSD+MVP Short (<100 m, 3 epochs) & $66.0$ ($72.8$)& $53.0$ ($66.3$)& $20.9$ ($38.8$)& $43.1$ ($54.0$)& $28.4$ ($44.1$)& $25.7$ ($42.2$)& $7.3$ ($23.1$)& $16.9$ ($30.8$) \\ 
 & FSD+MVP (3 epochs) & $66.0$ ($72.8$)& $52.8$ ($66.2$)& $18.7$ ($37.2$)& $42.0$ ($53.7$)& $28.0$ ($44.3$)& $24.4$ ($39.8$)& $7.1$ ($22.8$)& $16.6$ ($30.7$) \\ 
 \hline 
 \multirow{4}{*}{150 m}& FSD (6 epochs) & $29.2$ ($42.7$)& $14.7$ ($30.2$)& $0.5$ ($2.9$)& $7.9$ ($22.2$)& $2.3$ ($11.2$)& $8.2$ ($21.8$)& $1.2$ ($11.2$)& $4.1$ ($11.8$) \\ 
 & FSD+MVP Long (0-250m with range weights, 3 epochs)  & $39.6$ ($52.2$)& $21.4$ ($38.4$)& $1.7$ ($10.4$)& $10.9$ ($27.5$)& $4.9$ ($15.4$)& $10.4$ ($26.1$)& $2.2$ ($17.2$)& $5.7$ ($14.7$) \\ 
 & FSD+MVP Short (<100 m, 3 epochs) & $2.9$ ($3.4$)& $0.2$ ($0.0$)& $0.0$ ($0.0$)& $0.0$ ($0.0$)& $0.0$ ($0.0$)& $1.2$ ($2.4$)& $0.2$ ($1.1$)& $0.5$ ($0.8$) \\ 
 & FSD+MVP (3 epochs) & $39.2$ ($52.3$)& $21.6$ ($38.2$)& $2.0$ ($8.8$)& $11.2$ ($27.2$)& $3.7$ ($14.6$)& $10.0$ ($25.3$)& $2.1$ ($16.3$)& $5.4$ ($14.6$) \\ 
 \hline 
 \multirow{4}{*}{200 m}& FSD (6 epochs) & $13.9$ ($27.9$)& $1.2$ ($3.4$)& $0.0$ ($0.0$)& $1.1$ ($3.2$)& $0.0$ ($0.0$)& $2.6$ ($10.6$)& $2.0$ ($8.8$)& $1.0$ ($3.9$) \\ 
 & FSD+MVP Long (0-250m with range weights, 3 epochs)  & $22.6$ ($38.1$)& $6.1$ ($13.9$)& $0.0$ ($0.0$)& $2.2$ ($7.0$)& $0.2$ ($0.1$)& $4.5$ ($15.3$)& $3.5$ ($13.4$)& $1.8$ ($5.9$) \\ 
 & FSD+MVP Short (<100 m, 3 epochs) & $ - $& $ - $& $ - $& $ - $& $ - $& $ - $& $ - $& $ - $ \\ 
 & FSD+MVP (3 epochs) & $23.1$ ($38.6$)& $5.7$ ($12.4$)& $0.0$ ($0.0$)& $1.9$ ($6.0$)& $0.0$ ($0.0$)& $3.0$ ($13.2$)& $3.5$ ($13.3$)& $1.8$ ($5.5$) \\ 
 \hline 
 \multirow{4}{*}{250 m}& FSD (6 epochs) & $3.6$ ($9.0$)& $0.0$ ($0.0$)& $0.0$ ($0.0$)& $0.0$ ($0.0$)& $0.0$ ($0.0$)& $2.5$ ($4.1$)& $0.4$ ($1.9$)& $0.3$ ($0.8$) \\ 
 & FSD+MVP Long (0-250m with range weights, 3 epochs)  & $6.2$ ($13.1$)& $0.0$ ($0.0$)& $0.0$ ($0.0$)& $0.0$ ($0.0$)& $0.0$ ($0.0$)& $2.9$ ($4.9$)& $0.7$ ($3.3$)& $0.4$ ($1.1$) \\ 
 & FSD+MVP Short (<100 m, 3 epochs) & $ - $& $ - $& $ - $& $ - $& $ - $& $ - $& $ - $& $ - $ \\ 
 & FSD+MVP (3 epochs) & $6.0$ ($14.0$)& $0.0$ ($0.0$)& $0.0$ ($0.0$)& $0.0$ ($0.0$)& $0.0$ ($0.0$)& $3.5$ ($5.4$)& $0.6$ ($3.6$)& $0.5$ ($1.3$) \\ 
 \hline 
 \hline 
\end{tabular} 
\end{table*} 


==> tables/Custom_Table_AP.tex <==
\begin{table*}[t] 
\centering 
\footnotesize 
\caption{The AP are reported for the different classes, methods and ranges.} 
 
\setlength{\tabcolsep}{2pt}\begin{tabular}{ll|cccccccc} 
 
 \hline 
 Range & Method  & \rot{Vehicle } & \rot{Pedestrian } & \rot{Const. Cone } & \rot{Constr. Barrel } & \rot{Bollard } & \rot{Box Truck } & \rot{Large Vehicle } & \rot{Average All Classes }\\ 
\hline 
\multirow{4}{*}{0-250 m}& FSD (6 epochs) & $71.5$& $66.4$& $45.6$& $52.7$& $51.5$& $37.3$& $5.6$& $29.8$ \\ 
 & FSD+MVP Long (range weights, 3 epochs)  & $74.3$& $68.7$& $54.2$& $57.8$& $51.9$& $38.7$& $5.6$& $31.3$ \\ 
 & FSD+MVP Short (<100 m, 3 epochs) & $68.1$& $67.0$& $54.5$& $56.2$& $53.0$& $37.0$& $5.6$& $31.2$ \\ 
 & FSD+MVP (3 epochs) & $74.5$& $69.1$& $53.2$& $57.5$& $52.3$& $38.0$& $5.7$& $31.5$ \\ 
 \hline 
 \multirow{4}{*}{50 m}& FSD (6 epochs) & $89.0$& $82.0$& $59.6$& $79.6$& $66.0$& $64.2$& $10.7$& $44.9$ \\ 
 & FSD+MVP Long (range weights, 3 epochs)  & $88.9$& $82.5$& $68.1$& $82.9$& $65.2$& $63.9$& $10.0$& $45.9$ \\ 
 & FSD+MVP Short (<100 m, 3 epochs) & $89.2$& $82.9$& $68.6$& $83.4$& $67.0$& $65.3$& $11.2$& $46.9$ \\ 
 & FSD+MVP (3 epochs) & $89.0$& $82.9$& $67.1$& $82.3$& $65.8$& $64.5$& $9.8$& $46.4$ \\ 
 \hline 
 \multirow{4}{*}{100 m}& FSD (6 epochs) & $61.7$& $46.0$& $9.6$& $32.4$& $23.5$& $24.0$& $5.9$& $14.3$ \\ 
 & FSD+MVP Long (range weights, 3 epochs)  & $65.8$& $52.8$& $20.6$& $41.6$& $28.3$& $27.2$& $7.3$& $17.0$ \\ 
 & FSD+MVP Short (<100 m, 3 epochs) & $66.0$& $53.0$& $20.9$& $43.1$& $28.4$& $25.7$& $7.3$& $16.9$ \\ 
 & FSD+MVP (3 epochs) & $66.0$& $52.8$& $18.7$& $42.0$& $28.0$& $24.4$& $7.1$& $16.6$ \\ 
 \hline 
 \multirow{4}{*}{150 m}& FSD (6 epochs) & $29.2$& $14.7$& $0.5$& $7.9$& $2.3$& $8.2$& $1.2$& $4.1$ \\ 
 & FSD+MVP Long (range weights, 3 epochs)  & $39.6$& $21.4$& $1.7$& $10.9$& $4.9$& $10.4$& $2.2$& $5.7$ \\ 
 & FSD+MVP Short (<100 m, 3 epochs) & $2.9$& $0.2$& $0.0$& $0.0$& $0.0$& $1.2$& $0.2$& $0.5$ \\ 
 & FSD+MVP (3 epochs) & $39.2$& $21.6$& $2.0$& $11.2$& $3.7$& $10.0$& $2.1$& $5.4$ \\ 
 \hline 
 \multirow{4}{*}{200 m}& FSD (6 epochs) & $13.9$& $1.2$& $0.0$& $1.1$& $0.0$& $2.6$& $2.0$& $1.0$ \\ 
 & FSD+MVP Long (range weights, 3 epochs)  & $22.6$& $6.1$& $0.0$& $2.2$& $0.2$& $4.5$& $3.5$& $1.8$ \\ 
 & FSD+MVP Short (<100 m, 3 epochs) & $ - $& $ - $& $ - $& $ - $& $ - $& $ - $& $ - $& $ - $ \\ 
 & FSD+MVP (3 epochs) & $23.1$& $5.7$& $0.0$& $1.9$& $0.0$& $3.0$& $3.5$& $1.8$ \\ 
 \hline 
 \multirow{4}{*}{250 m}& FSD (6 epochs) & $3.6$& $0.0$& $0.0$& $0.0$& $0.0$& $2.5$& $0.4$& $0.3$ \\ 
 & FSD+MVP Long (range weights, 3 epochs)  & $6.2$& $0.0$& $0.0$& $0.0$& $0.0$& $2.9$& $0.7$& $0.4$ \\ 
 & FSD+MVP Short (<100 m, 3 epochs) & $ - $& $ - $& $ - $& $ - $& $ - $& $ - $& $ - $& $ - $ \\ 
 & FSD+MVP (3 epochs) & $6.0$& $0.0$& $0.0$& $0.0$& $0.0$& $3.5$& $0.6$& $0.5$ \\ 
 \hline 
 \hline 
\end{tabular} 
\end{table*} 


==> tables/Custom_Table_AR.tex <==
\begin{table*}[t] 
\centering 
\footnotesize 
\caption{The AR are reported for the different classes, methods and ranges.} 
 
\setlength{\tabcolsep}{2pt}\begin{tabular}{ll|cccccccc} 
 
 \hline 
 Range & Method  & \rot{Vehicle } & \rot{Pedestrian } & \rot{Const. Cone } & \rot{Constr. Barrel } & \rot{Bollard } & \rot{Box Truck } & \rot{Large Vehicle } & \rot{Average All Classes }\\ 
\hline 
\multirow{4}{*}{0-250 m}& FSD (6 epochs) & $75.4$& $72.2$& $54.9$& $58.8$& $61.4$& $46.6$& $19.4$& $42.1$ \\ 
 & FSD+MVP Long (range weights, 3 epochs)  & $78.1$& $74.7$& $63.1$& $63.8$& $62.3$& $48.8$& $22.6$& $43.9$ \\ 
 & FSD+MVP Short (<100 m, 3 epochs) & $70.7$& $71.8$& $62.3$& $60.3$& $61.9$& $44.9$& $17.9$& $41.7$ \\ 
 & FSD+MVP (3 epochs) & $78.3$& $74.8$& $62.0$& $63.5$& $62.1$& $47.7$& $20.9$& $43.4$ \\ 
 \hline 
 \multirow{4}{*}{50 m}& FSD (6 epochs) & $91.3$& $86.0$& $68.9$& $83.8$& $75.0$& $72.9$& $35.1$& $59.3$ \\ 
 & FSD+MVP Long (range weights, 3 epochs)  & $91.4$& $86.5$& $76.2$& $86.4$& $74.6$& $73.1$& $37.1$& $59.9$ \\ 
 & FSD+MVP Short (<100 m, 3 epochs) & $91.6$& $86.8$& $75.8$& $86.6$& $75.4$& $74.1$& $36.6$& $59.5$ \\ 
 & FSD+MVP (3 epochs) & $91.5$& $86.7$& $75.2$& $85.7$& $74.7$& $73.5$& $34.7$& $59.4$ \\ 
 \hline 
 \multirow{4}{*}{100 m}& FSD (6 epochs) & $69.1$& $60.8$& $26.5$& $44.2$& $41.2$& $39.0$& $20.2$& $28.2$ \\ 
 & FSD+MVP Long (range weights, 3 epochs)  & $72.5$& $66.1$& $38.7$& $53.3$& $44.7$& $42.3$& $25.6$& $31.5$ \\ 
 & FSD+MVP Short (<100 m, 3 epochs) & $72.8$& $66.3$& $38.8$& $54.0$& $44.1$& $42.2$& $23.1$& $30.8$ \\ 
 & FSD+MVP (3 epochs) & $72.8$& $66.2$& $37.2$& $53.7$& $44.3$& $39.8$& $22.8$& $30.7$ \\ 
 \hline 
 \multirow{4}{*}{150 m}& FSD (6 epochs) & $42.7$& $30.2$& $2.9$& $22.2$& $11.2$& $21.8$& $11.2$& $11.8$ \\ 
 & FSD+MVP Long (range weights, 3 epochs)  & $52.2$& $38.4$& $10.4$& $27.5$& $15.4$& $26.1$& $17.2$& $14.7$ \\ 
 & FSD+MVP Short (<100 m, 3 epochs) & $3.4$& $0.0$& $0.0$& $0.0$& $0.0$& $2.4$& $1.1$& $0.8$ \\ 
 & FSD+MVP (3 epochs) & $52.3$& $38.2$& $8.8$& $27.2$& $14.6$& $25.3$& $16.3$& $14.6$ \\ 
 \hline 
 \multirow{4}{*}{200 m}& FSD (6 epochs) & $27.9$& $3.4$& $0.0$& $3.2$& $0.0$& $10.6$& $8.8$& $3.9$ \\ 
 & FSD+MVP Long (range weights, 3 epochs)  & $38.1$& $13.9$& $0.0$& $7.0$& $0.1$& $15.3$& $13.4$& $5.9$ \\ 
 & FSD+MVP Short (<100 m, 3 epochs) & $ - $& $ - $& $ - $& $ - $& $ - $& $ - $& $ - $& $ - $ \\ 
 & FSD+MVP (3 epochs) & $38.6$& $12.4$& $0.0$& $6.0$& $0.0$& $13.2$& $13.3$& $5.5$ \\ 
 \hline 
 \multirow{4}{*}{250 m}& FSD (6 epochs) & $9.0$& $0.0$& $0.0$& $0.0$& $0.0$& $4.1$& $1.9$& $0.8$ \\ 
 & FSD+MVP Long (range weights, 3 epochs)  & $13.1$& $0.0$& $0.0$& $0.0$& $0.0$& $4.9$& $3.3$& $1.1$ \\ 
 & FSD+MVP Short (<100 m, 3 epochs) & $ - $& $ - $& $ - $& $ - $& $ - $& $ - $& $ - $& $ - $ \\ 
 & FSD+MVP (3 epochs) & $14.0$& $0.0$& $0.0$& $0.0$& $0.0$& $5.4$& $3.6$& $1.3$ \\ 
 \hline 
 \hline 
\end{tabular} 
\end{table*} 


==> tables/Custom_Table_Experiments_AP.tex <==
\begin{table*}[t] 
\centering 
\caption{The AP are reported for the different classes, methods and ranges.} 

%\setlength{\tabcolsep}{2pt}
\begin{tabular}{l|cccccc} 
 
 \hline 
 Method  & \rot{0-250 m} & \rot{0-50 m} & \rot{50-100 m} & \rot{100-150 m} & \rot{150-200 m} & \rot{200-250 m}\\ 
\hline 
FSD (6 epochs) & $29.8$& $44.9$& $14.3$& $4.1$& $1.0$& $0.3$ \\ 
 FSD+MVP (3 epochs) & $31.5$& $46.4$& $16.6$& $5.4$& $1.8$& $0.5$ \\ 
 FSD+MVP Short (<100 m, 3 epochs) & $31.2$& $46.9$& $16.9$& $0.5$& $ - $& $ - $ \\ 
 FSD+MVP Long (range weights, 3 epochs)  & $31.3$& $45.9$& $17.0$& $5.7$& $1.8$& $0.4$ \\ 
 
 \hline 
\end{tabular} 
\end{table*} 


==> tables/Custom_Table_all.tex <==
\begin{table*}[t] 
\centering 
\footnotesize 
\caption{The AP are reported for the different classes, methods and ranges.} 
 
\setlength{\tabcolsep}{2pt}\begin{tabular}{ll|ccccccccccccccccccccccccccc} 
 
 \hline 
 Range & Method  & \rot{Articulated Bus } & \rot{Bicycle } & \rot{Bicyclist } & \rot{Bollard } & \rot{Box Truck } & \rot{Bus } & \rot{Constr. Barrel } & \rot{Const. Cone } & \rot{Dog } & \rot{Large Vehicle } & \rot{Message Board Trailer } & \rot{M. Ped. Cross. Sign } & \rot{Motorcyle } & \rot{Motorcyclist } & \rot{Pedestrian } & \rot{Vehicle } & \rot{School Bus } & \rot{Sign } & \rot{Stop Sign } & \rot{Stroller } & \rot{Truck } & \rot{Truck Cab } & \rot{Trailer } & \rot{Wheelchair } & \rot{Wheeled Device } & \rot{Wheeled Rider } & \rot{Average All Classes }\\ 
\hline 
\multirow{3}{*}{0-250 m}& Default & $19.3$& $37.9$& $34.1$& $46.9$& $37.7$& $40.8$& $44.4$& $43.7$& $10.2$& $5.8$& $0.0$& $26.5$& $48.2$& $39.9$& $63.9$& $70.5$& $29.5$& $11.5$& $28.9$& $12.8$& $20.7$& $12.0$& $25.6$& $7.1$& $14.2$& $9.0$& $28.5$ \\ 
 & IMFSD & $19.1$& $37.6$& $32.5$& $46.9$& $35.9$& $39.4$& $43.9$& $43.5$& $10.3$& $5.2$& $0.0$& $25.3$& $48.4$& $38.9$& $62.7$& $69.6$& $29.0$& $10.6$& $28.6$& $12.8$& $20.3$& $17.7$& $24.7$& $6.6$& $14.2$& $8.7$& $28.2$ \\ 
 & Default+MVP & $17.2$& $38.7$& $35.2$& $49.4$& $37.6$& $40.8$& $48.6$& $44.3$& $2.4$& $5.3$& $0.0$& $25.1$& $49.2$& $36.9$& $66.0$& $72.5$& $28.6$& $10.7$& $29.2$& $9.1$& $21.0$& $17.6$& $26.9$& $0.9$& $15.0$& $8.1$& $28.3$ \\ 
 \hline 
 \multirow{3}{*}{50 m}& Default & $33.5$& $50.0$& $59.8$& $62.3$& $65.5$& $69.0$& $73.7$& $58.0$& $12.1$& $11.6$& $0.0$& $54.2$& $63.6$& $63.4$& $81.0$& $88.9$& $72.2$& $19.8$& $50.1$& $16.9$& $29.4$& $17.5$& $40.5$& $9.9$& $19.4$& $14.1$& $43.7$ \\ 
 & IMFSD & $33.9$& $49.7$& $57.1$& $62.3$& $64.4$& $67.6$& $72.8$& $57.7$& $12.3$& $10.4$& $0.0$& $54.6$& $63.8$& $61.5$& $80.0$& $88.9$& $71.0$& $19.7$& $50.1$& $16.9$& $28.9$& $27.4$& $39.4$& $9.2$& $19.4$& $13.4$& $43.6$ \\ 
 & Default+MVP & $29.7$& $50.8$& $61.4$& $63.9$& $64.8$& $67.5$& $75.7$& $58.4$& $2.9$& $10.3$& $0.0$& $51.3$& $64.3$& $59.8$& $81.7$& $89.0$& $70.4$& $18.6$& $50.5$& $12.7$& $29.9$& $29.4$& $42.6$& $1.4$& $20.8$& $13.6$& $43.1$ \\ 
 \hline 
 \multirow{3}{*}{100 m}& Default & $5.7$& $9.2$& $19.7$& $16.3$& $23.7$& $30.6$& $19.4$& $7.0$& $2.7$& $5.3$& $0.0$& $10.6$& $9.8$& $8.0$& $40.9$& $59.7$& $9.4$& $4.0$& $3.5$& $0.0$& $18.1$& $10.0$& $12.1$& $1.5$& $0.4$& $1.5$& $12.6$ \\ 
 & IMFSD & $5.2$& $9.1$& $18.8$& $16.2$& $21.7$& $29.8$& $18.8$& $6.7$& $3.0$& $5.1$& $0.0$& $10.5$& $10.0$& $7.7$& $40.2$& $59.5$& $9.2$& $4.0$& $3.4$& $0.0$& $18.1$& $11.9$& $12.4$& $1.7$& $0.4$& $1.5$& $12.5$ \\ 
 & Default+MVP & $6.2$& $9.9$& $20.5$& $21.0$& $23.5$& $31.1$& $26.6$& $7.5$& $0.6$& $5.1$& $0.1$& $9.4$& $9.7$& $7.7$& $44.0$& $60.5$& $9.7$& $3.4$& $3.3$& $0.0$& $18.6$& $8.0$& $11.7$& $0.1$& $0.3$& $1.4$& $13.1$ \\ 
 \hline 
 \multirow{3}{*}{150 m}& Default & $4.5$& $0.4$& $1.5$& $1.9$& $8.4$& $15.3$& $1.0$& $0.1$& $0.0$& $1.2$& $0.0$& $0.1$& $0.1$& $0.2$& $11.2$& $26.8$& $0.3$& $0.4$& $0.4$& $0.0$& $4.7$& $2.5$& $4.5$& $0.0$& $0.5$& $0.0$& $3.3$ \\ 
 & IMFSD & $3.6$& $0.4$& $1.5$& $1.5$& $7.3$& $12.0$& $1.8$& $0.1$& $0.0$& $1.2$& $0.0$& $0.1$& $0.1$& $0.2$& $8.1$& $22.5$& $0.8$& $0.4$& $0.3$& $0.0$& $4.6$& $4.4$& $2.7$& $0.0$& $0.4$& $0.0$& $2.8$ \\ 
 & Default+MVP & $2.2$& $1.3$& $1.0$& $2.9$& $9.4$& $16.7$& $6.3$& $2.6$& $0.0$& $2.4$& $0.0$& $0.1$& $2.2$& $1.2$& $18.6$& $37.4$& $0.2$& $0.3$& $0.2$& $0.0$& $3.6$& $1.6$& $3.2$& $0.0$& $0.0$& $0.0$& $4.4$ \\ 
 \hline 
 \multirow{3}{*}{200 m}& Default & $0.2$& $0.0$& $0.2$& $0.0$& $3.3$& $0.9$& $0.1$& $0.0$& $0.0$& $2.3$& $0.0$& $0.0$& $0.0$& $0.0$& $1.1$& $12.1$& $0.1$& $1.1$& $0.1$& $0.0$& $0.8$& $3.7$& $0.2$& $0.0$& $0.0$& $0.0$& $1.0$ \\ 
 & IMFSD & $0.2$& $0.0$& $0.1$& $2.2$& $1.8$& $1.1$& $0.5$& $0.0$& $0.0$& $2.3$& $0.0$& $0.0$& $0.0$& $0.0$& $1.2$& $9.6$& $0.1$& $0.1$& $0.1$& $0.0$& $1.0$& $3.7$& $0.2$& $0.0$& $0.0$& $0.0$& $0.9$ \\ 
 & Default+MVP & $0.0$& $0.0$& $0.1$& $0.5$& $4.6$& $3.3$& $2.2$& $0.0$& $0.0$& $3.8$& $0.0$& $0.0$& $0.0$& $0.0$& $4.9$& $22.1$& $0.0$& $0.3$& $0.1$& $0.0$& $0.6$& $1.4$& $0.7$& $0.0$& $0.0$& $0.0$& $1.7$ \\ 
 \hline 
 \multirow{3}{*}{250 m}& Default & $0.0$& $0.0$& $0.0$& $0.0$& $1.3$& $0.0$& $0.0$& $0.0$& $0.0$& $0.6$& $0.0$& $0.0$& $0.0$& $0.0$& $0.0$& $2.7$& $0.0$& $0.0$& $0.0$& $0.0$& $2.7$& $1.3$& $0.0$& $0.0$& $0.0$& $0.0$& $0.3$ \\ 
 & IMFSD & $0.0$& $0.0$& $0.0$& $0.0$& $0.9$& $0.0$& $0.0$& $0.0$& $0.0$& $0.4$& $0.0$& $0.0$& $0.0$& $0.0$& $0.1$& $2.8$& $0.0$& $0.0$& $0.3$& $0.0$& $2.7$& $1.3$& $0.0$& $0.0$& $0.0$& $0.0$& $0.3$ \\ 
 & Default+MVP & $0.0$& $0.0$& $0.0$& $0.0$& $3.6$& $0.1$& $0.0$& $0.0$& $0.0$& $1.5$& $0.0$& $0.0$& $0.0$& $0.0$& $0.0$& $6.5$& $0.0$& $1.0$& $0.0$& $0.0$& $0.3$& $1.5$& $0.4$& $0.0$& $0.0$& $0.0$& $0.6$ \\ 
 \hline 
 \hline 
\end{tabular} 
\end{table*} 


==> tables/Custom_Table_all_AP.tex <==
\begin{table*}[t] 
\centering 
\footnotesize 
\caption{The AP are reported for the different classes, methods and ranges.} 
 
\setlength{\tabcolsep}{2pt}\begin{tabular}{ll|ccccccccccccccccccccccccccc} 
 
 \hline 
 Range & Method  & \rot{Articulated Bus } & \rot{Bicycle } & \rot{Bicyclist } & \rot{Bollard } & \rot{Box Truck } & \rot{Bus } & \rot{Constr. Barrel } & \rot{Const. Cone } & \rot{Dog } & \rot{Large Vehicle } & \rot{Message Board Trailer } & \rot{M. Ped. Cross. Sign } & \rot{Motorcyle } & \rot{Motorcyclist } & \rot{Pedestrian } & \rot{Vehicle } & \rot{School Bus } & \rot{Sign } & \rot{Stop Sign } & \rot{Stroller } & \rot{Truck } & \rot{Truck Cab } & \rot{Trailer } & \rot{Wheelchair } & \rot{Wheeled Device } & \rot{Wheeled Rider } & \rot{Average All Classes }\\ 
\hline 
\multirow{3}{*}{0-250 m}& Default & $19.3$& $37.9$& $34.1$& $46.9$& $37.7$& $40.8$& $44.4$& $43.7$& $10.2$& $5.8$& $0.0$& $26.5$& $48.2$& $39.9$& $63.9$& $70.5$& $29.5$& $11.5$& $28.9$& $12.8$& $20.7$& $12.0$& $25.6$& $7.1$& $14.2$& $9.0$& $28.5$ \\ 
 & IMFSD & $19.1$& $37.6$& $32.5$& $46.9$& $35.9$& $39.4$& $43.9$& $43.5$& $10.3$& $5.2$& $0.0$& $25.3$& $48.4$& $38.9$& $62.7$& $69.6$& $29.0$& $10.6$& $28.6$& $12.8$& $20.3$& $17.7$& $24.7$& $6.6$& $14.2$& $8.7$& $28.2$ \\ 
 & Default+MVP & $17.2$& $38.7$& $35.2$& $49.4$& $37.6$& $40.8$& $48.6$& $44.3$& $2.4$& $5.3$& $0.0$& $25.1$& $49.2$& $36.9$& $66.0$& $72.5$& $28.6$& $10.7$& $29.2$& $9.1$& $21.0$& $17.6$& $26.9$& $0.9$& $15.0$& $8.1$& $28.3$ \\ 
 \hline 
 \multirow{3}{*}{50 m}& Default & $33.5$& $50.0$& $59.8$& $62.3$& $65.5$& $69.0$& $73.7$& $58.0$& $12.1$& $11.6$& $0.0$& $54.2$& $63.6$& $63.4$& $81.0$& $88.9$& $72.2$& $19.8$& $50.1$& $16.9$& $29.4$& $17.5$& $40.5$& $9.9$& $19.4$& $14.1$& $43.7$ \\ 
 & IMFSD & $33.9$& $49.7$& $57.1$& $62.3$& $64.4$& $67.6$& $72.8$& $57.7$& $12.3$& $10.4$& $0.0$& $54.6$& $63.8$& $61.5$& $80.0$& $88.9$& $71.0$& $19.7$& $50.1$& $16.9$& $28.9$& $27.4$& $39.4$& $9.2$& $19.4$& $13.4$& $43.6$ \\ 
 & Default+MVP & $29.7$& $50.8$& $61.4$& $63.9$& $64.8$& $67.5$& $75.7$& $58.4$& $2.9$& $10.3$& $0.0$& $51.3$& $64.3$& $59.8$& $81.7$& $89.0$& $70.4$& $18.6$& $50.5$& $12.7$& $29.9$& $29.4$& $42.6$& $1.4$& $20.8$& $13.6$& $43.1$ \\ 
 \hline 
 \multirow{3}{*}{100 m}& Default & $5.7$& $9.2$& $19.7$& $16.3$& $23.7$& $30.6$& $19.4$& $7.0$& $2.7$& $5.3$& $0.0$& $10.6$& $9.8$& $8.0$& $40.9$& $59.7$& $9.4$& $4.0$& $3.5$& $0.0$& $18.1$& $10.0$& $12.1$& $1.5$& $0.4$& $1.5$& $12.6$ \\ 
 & IMFSD & $5.2$& $9.1$& $18.8$& $16.2$& $21.7$& $29.8$& $18.8$& $6.7$& $3.0$& $5.1$& $0.0$& $10.5$& $10.0$& $7.7$& $40.2$& $59.5$& $9.2$& $4.0$& $3.4$& $0.0$& $18.1$& $11.9$& $12.4$& $1.7$& $0.4$& $1.5$& $12.5$ \\ 
 & Default+MVP & $6.2$& $9.9$& $20.5$& $21.0$& $23.5$& $31.1$& $26.6$& $7.5$& $0.6$& $5.1$& $0.1$& $9.4$& $9.7$& $7.7$& $44.0$& $60.5$& $9.7$& $3.4$& $3.3$& $0.0$& $18.6$& $8.0$& $11.7$& $0.1$& $0.3$& $1.4$& $13.1$ \\ 
 \hline 
 \multirow{3}{*}{150 m}& Default & $4.5$& $0.4$& $1.5$& $1.9$& $8.4$& $15.3$& $1.0$& $0.1$& $0.0$& $1.2$& $0.0$& $0.1$& $0.1$& $0.2$& $11.2$& $26.8$& $0.3$& $0.4$& $0.4$& $0.0$& $4.7$& $2.5$& $4.5$& $0.0$& $0.5$& $0.0$& $3.3$ \\ 
 & IMFSD & $3.6$& $0.4$& $1.5$& $1.5$& $7.3$& $12.0$& $1.8$& $0.1$& $0.0$& $1.2$& $0.0$& $0.1$& $0.1$& $0.2$& $8.1$& $22.5$& $0.8$& $0.4$& $0.3$& $0.0$& $4.6$& $4.4$& $2.7$& $0.0$& $0.4$& $0.0$& $2.8$ \\ 
 & Default+MVP & $2.2$& $1.3$& $1.0$& $2.9$& $9.4$& $16.7$& $6.3$& $2.6$& $0.0$& $2.4$& $0.0$& $0.1$& $2.2$& $1.2$& $18.6$& $37.4$& $0.2$& $0.3$& $0.2$& $0.0$& $3.6$& $1.6$& $3.2$& $0.0$& $0.0$& $0.0$& $4.4$ \\ 
 \hline 
 \multirow{3}{*}{200 m}& Default & $0.2$& $0.0$& $0.2$& $0.0$& $3.3$& $0.9$& $0.1$& $0.0$& $0.0$& $2.3$& $0.0$& $0.0$& $0.0$& $0.0$& $1.1$& $12.1$& $0.1$& $1.1$& $0.1$& $0.0$& $0.8$& $3.7$& $0.2$& $0.0$& $0.0$& $0.0$& $1.0$ \\ 
 & IMFSD & $0.2$& $0.0$& $0.1$& $2.2$& $1.8$& $1.1$& $0.5$& $0.0$& $0.0$& $2.3$& $0.0$& $0.0$& $0.0$& $0.0$& $1.2$& $9.6$& $0.1$& $0.1$& $0.1$& $0.0$& $1.0$& $3.7$& $0.2$& $0.0$& $0.0$& $0.0$& $0.9$ \\ 
 & Default+MVP & $0.0$& $0.0$& $0.1$& $0.5$& $4.6$& $3.3$& $2.2$& $0.0$& $0.0$& $3.8$& $0.0$& $0.0$& $0.0$& $0.0$& $4.9$& $22.1$& $0.0$& $0.3$& $0.1$& $0.0$& $0.6$& $1.4$& $0.7$& $0.0$& $0.0$& $0.0$& $1.7$ \\ 
 \hline 
 \multirow{3}{*}{250 m}& Default & $0.0$& $0.0$& $0.0$& $0.0$& $1.3$& $0.0$& $0.0$& $0.0$& $0.0$& $0.6$& $0.0$& $0.0$& $0.0$& $0.0$& $0.0$& $2.7$& $0.0$& $0.0$& $0.0$& $0.0$& $2.7$& $1.3$& $0.0$& $0.0$& $0.0$& $0.0$& $0.3$ \\ 
 & IMFSD & $0.0$& $0.0$& $0.0$& $0.0$& $0.9$& $0.0$& $0.0$& $0.0$& $0.0$& $0.4$& $0.0$& $0.0$& $0.0$& $0.0$& $0.1$& $2.8$& $0.0$& $0.0$& $0.3$& $0.0$& $2.7$& $1.3$& $0.0$& $0.0$& $0.0$& $0.0$& $0.3$ \\ 
 & Default+MVP & $0.0$& $0.0$& $0.0$& $0.0$& $3.6$& $0.1$& $0.0$& $0.0$& $0.0$& $1.5$& $0.0$& $0.0$& $0.0$& $0.0$& $0.0$& $6.5$& $0.0$& $1.0$& $0.0$& $0.0$& $0.3$& $1.5$& $0.4$& $0.0$& $0.0$& $0.0$& $0.6$ \\ 
 \hline 
 \hline 
\end{tabular} 
\end{table*} 


==> tables/Custom_Table_all_AR.tex <==
\begin{table*}[t] 
\centering 
\tiny 
\caption{The AR are reported for the different classes, methods and ranges.} 
 
\setlength{\tabcolsep}{2pt}\begin{tabular}{ll|ccccccccccccccccccccccccccc} 
 
 \hline 
 Range & Method  & \rot{Articulated Bus } & \rot{Bicycle } & \rot{Bicyclist } & \rot{Bollard } & \rot{Box Truck } & \rot{Bus } & \rot{Constr. Barrel } & \rot{Const. Cone } & \rot{Dog } & \rot{Large Vehicle } & \rot{Message Board Trailer } & \rot{M. Ped. Cross. Sign } & \rot{Motorcyle } & \rot{Motorcyclist } & \rot{Pedestrian } & \rot{Vehicle } & \rot{School Bus } & \rot{Sign } & \rot{Stop Sign } & \rot{Stroller } & \rot{Truck } & \rot{Truck Cab } & \rot{Trailer } & \rot{Wheelchair } & \rot{Wheeled Device } & \rot{Wheeled Rider } & \rot{Average All Classes }\\ 
\hline 
\multirow{3}{*}{0-250 m}& Default & $31.9$& $49.6$& $48.5$& $59.2$& $47.3$& $49.1$& $50.9$& $53.4$& $28.4$& $20.2$& $0.0$& $43.0$& $60.1$& $63.2$& $70.6$& $74.3$& $36.7$& $30.1$& $40.5$& $41.2$& $42.1$& $20.3$& $33.1$& $19.4$& $28.7$& $23.5$& $41.0$ \\ 
 & IMFSD & $32.8$& $50.0$& $48.7$& $59.2$& $47.4$& $49.8$& $51.2$& $53.7$& $29.2$& $20.8$& $0.0$& $43.4$& $60.9$& $63.6$& $70.6$& $74.6$& $38.2$& $30.3$& $40.4$& $41.2$& $44.6$& $28.6$& $33.9$& $20.4$& $28.9$& $23.8$& $41.8$ \\ 
 & Default+MVP & $27.7$& $50.7$& $49.8$& $60.5$& $47.3$& $49.6$& $55.1$& $54.0$& $28.9$& $21.8$& $9.9$& $40.7$& $60.6$& $62.6$& $72.3$& $76.4$& $35.7$& $29.8$& $40.8$& $41.6$& $43.2$& $26.4$& $34.0$& $19.2$& $29.7$& $22.3$& $41.9$ \\ 
 \hline 
 \multirow{3}{*}{50 m}& Default & $47.0$& $63.8$& $73.6$& $73.9$& $75.0$& $75.8$& $79.6$& $68.3$& $34.0$& $37.7$& $0.0$& $73.6$& $75.4$& $84.0$& $85.5$& $91.3$& $79.0$& $46.5$& $64.7$& $53.7$& $54.1$& $25.6$& $50.0$& $27.8$& $38.3$& $33.2$& $58.1$ \\ 
 & IMFSD & $48.8$& $64.1$& $74.1$& $73.9$& $75.1$& $76.2$& $79.9$& $68.7$& $34.8$& $39.0$& $0.0$& $75.8$& $76.4$& $84.2$& $85.5$& $91.3$& $80.2$& $46.7$& $64.7$& $53.5$& $56.8$& $38.8$& $50.7$& $29.1$& $38.6$& $33.4$& $59.2$ \\ 
 & Default+MVP & $40.7$& $64.6$& $74.7$& $74.2$& $74.2$& $74.6$& $80.7$& $68.3$& $34.3$& $36.7$& $0.0$& $70.7$& $75.5$& $81.0$& $85.8$& $91.4$& $78.5$& $45.9$& $65.2$& $54.9$& $55.6$& $37.2$& $51.1$& $27.1$& $39.3$& $31.4$& $58.2$ \\ 
 \hline 
 \multirow{3}{*}{100 m}& Default & $20.2$& $21.8$& $44.5$& $36.6$& $38.5$& $45.2$& $32.7$& $22.1$& $7.0$& $21.8$& $0.0$& $22.5$& $33.6$& $57.2$& $57.3$& $67.2$& $23.9$& $22.8$& $17.5$& $1.6$& $42.6$& $20.5$& $21.5$& $2.0$& $4.0$& $12.4$& $26.8$ \\ 
 & IMFSD & $21.4$& $22.1$& $44.7$& $36.6$& $38.4$& $46.3$& $33.0$& $22.1$& $7.2$& $22.6$& $0.0$& $22.8$& $34.7$& $58.2$& $57.4$& $67.3$& $26.5$& $23.1$& $17.6$& $1.6$& $46.6$& $24.8$& $23.8$& $2.0$& $4.1$& $12.9$& $27.6$ \\ 
 & Default+MVP & $18.5$& $22.7$& $44.8$& $40.2$& $37.6$& $45.5$& $38.7$& $23.2$& $11.5$& $21.7$& $10.5$& $20.9$& $31.5$& $55.5$& $59.0$& $67.7$& $22.1$& $22.8$& $18.1$& $1.7$& $42.6$& $19.1$& $21.5$& $6.0$& $5.6$& $8.9$& $27.6$ \\ 
 \hline 
 \multirow{3}{*}{150 m}& Default & $20.0$& $3.7$& $9.2$& $7.4$& $22.8$& $28.1$& $5.7$& $0.3$& $0.0$& $12.2$& $0.0$& $18.0$& $3.9$& $6.8$& $25.3$& $40.4$& $6.8$& $9.7$& $7.6$& $0.0$& $20.6$& $9.3$& $8.9$& $0.0$& $0.7$& $0.6$& $10.3$ \\ 
 & IMFSD & $20.1$& $3.7$& $9.5$& $7.4$& $23.3$& $29.4$& $5.8$& $0.3$& $0.0$& $12.4$& $0.0$& $19.3$& $3.9$& $6.8$& $25.7$& $42.0$& $8.0$& $12.2$& $8.6$& $0.0$& $22.4$& $13.1$& $9.2$& $0.0$& $0.7$& $0.6$& $10.9$ \\ 
 & Default+MVP & $12.2$& $8.2$& $12.8$& $11.0$& $23.5$& $30.8$& $17.8$& $7.1$& $0.0$& $18.2$& $0.0$& $12.3$& $11.0$& $14.0$& $36.9$& $51.3$& $5.9$& $8.4$& $4.6$& $4.2$& $25.4$& $10.8$& $8.1$& $0.0$& $0.3$& $0.6$& $12.9$ \\ 
 \hline 
 \multirow{3}{*}{200 m}& Default & $14.1$& $0.0$& $0.9$& $0.0$& $12.6$& $7.6$& $0.0$& $0.0$& $0.0$& $9.6$& $0.0$& $0.0$& $0.0$& $0.0$& $3.2$& $25.6$& $2.9$& $3.8$& $3.5$& $0.0$& $6.8$& $8.9$& $2.0$& $0.0$& $0.0$& $0.0$& $3.9$ \\ 
 & IMFSD & $14.1$& $0.0$& $0.9$& $3.7$& $13.6$& $8.7$& $0.1$& $0.0$& $0.0$& $10.5$& $0.0$& $0.0$& $0.0$& $0.0$& $7.1$& $32.6$& $3.0$& $4.0$& $6.0$& $0.0$& $8.4$& $11.0$& $2.5$& $0.0$& $0.0$& $0.0$& $4.9$ \\ 
 & Default+MVP & $3.9$& $0.5$& $1.3$& $0.3$& $16.1$& $13.5$& $4.1$& $0.0$& $0.0$& $16.5$& $0.0$& $0.0$& $0.0$& $0.0$& $14.6$& $39.1$& $1.2$& $3.9$& $2.7$& $0.0$& $10.3$& $11.3$& $5.5$& $0.0$& $0.0$& $0.0$& $5.6$ \\ 
 \hline 
 \multirow{3}{*}{250 m}& Default & $0.0$& $0.0$& $0.0$& $0.0$& $2.7$& $0.0$& $0.0$& $0.0$& $0.0$& $2.7$& $0.0$& $0.0$& $0.0$& $0.0$& $0.0$& $7.6$& $0.0$& $0.0$& $0.0$& $0.0$& $3.2$& $4.7$& $0.0$& $0.0$& $0.0$& $0.0$& $0.8$ \\ 
 & IMFSD & $0.0$& $0.0$& $0.0$& $0.0$& $2.6$& $0.8$& $0.0$& $0.0$& $0.0$& $2.8$& $0.0$& $0.0$& $0.0$& $0.0$& $0.3$& $15.0$& $0.0$& $0.5$& $5.3$& $0.0$& $3.2$& $4.7$& $0.0$& $0.0$& $0.0$& $0.0$& $1.3$ \\ 
 & Default+MVP & $0.0$& $0.0$& $0.0$& $0.0$& $6.0$& $1.9$& $0.0$& $0.0$& $0.0$& $4.8$& $0.0$& $0.0$& $0.0$& $0.0$& $0.0$& $15.7$& $0.0$& $2.0$& $0.0$& $0.0$& $4.5$& $7.1$& $0.4$& $0.0$& $0.0$& $0.0$& $1.6$ \\ 
 \hline 
 \hline 
\end{tabular} 
\end{table*} 


==> tables/Performance_breakdown.tex <==
\begin{table}[h] 
\centering 
\scriptsize
% \footnotesize 
\caption{Performance breakdown for different settings.} 
\label{tab:perf_breakdown}
\renewcommand{\arraystretch}{1.2}
 \setlength{\tabcolsep}{2pt}\begin{tabular}{l|c|c|ccccc}
 \hline 
  % \multirow{2}{*}{} &  MVP w/o  & MVP with & \multirow{2}{*}{} & \multirow{2}{*}{} & \multirow{2}{*}{} & \multirow{2}{*}{} & \multirow{2}{*}{} & \multirow{2}{*}{} \\
  
  Method  & MVP & 0-250 & 0-50 & 50-100 & 100-150 & 150-200 & 200-250 \\
 \hline
 \multirow{2}{*}{FSD} & $-$ & 29.8 & 44.9 & 14.3 & 4.1 & 1.0 & 0.3\\
 % & \checkmark & $-$ & 20.6 & 34.6 & 7.2 & 1.1 & 0.2 & 0.1\\
 &  \checkmark & 31.5 & 46.4 & 16.6 & 5.4 & 1.8 & 0.5\\
 \hline
 \multirow{2}{*}{RangeFSD} & $-$ & 30.2 & 45.5 & 14.8 & 4.6 & 1.2 & 0.3 \\
 %& \checkmark & $-$ & 20.7  & 34.9 & 7.2 & 1.0 & 0.3 & 0.1 \\
 & \checkmark & 31.9 & 46.9 & 16.9 & 5.8 & 2.0 & 0.5\\
 \hline 
\end{tabular} 
\end{table} 


%%%%%%%%%%% commented with and without finetuning part
% \begin{table}[h] 
% \centering 
% \scriptsize
% % \footnotesize 
% \caption{Performance breakdown for different settings.} 
% \label{tab:perf_breakdown}
% \renewcommand{\arraystretch}{1.2}
% % \setlength{\tabcolsep}{2pt}\begin{tabular}{l|c|c|c|c|c|c|c|c} 
%  \setlength{\tabcolsep}{2pt}\begin{tabular}{l|c|c|c|ccccc}
%  \hline 
%   \multirow{2}{*}{} &  MVP w/o  & MVP with & \multirow{2}{*}{} & \multirow{2}{*}{} & \multirow{2}{*}{} & \multirow{2}{*}{} & \multirow{2}{*}{} & \multirow{2}{*}{} \\
%   Method  & finetuning & finetuning & 0-250 & 0-50 & 50-100 & 100-150 & 150-200 & 200-250 \\
%  \hline
%  \multirow{3}{*}{FSD} & $-$ & $-$ & 29.8 & 44.9 & 14.3 & 4.1 & 1.0 & 0.3\\
%  & \checkmark & $-$ & 20.6 & 34.6 & 7.2 & 1.1 & 0.2 & 0.1\\
%  & $-$ & \checkmark & 31.5 & 46.4 & 16.6 & 5.4 & 1.8 & 0.5\\
%  \hline
%  \multirow{3}{*}{RangeFSD} & $-$ & $-$ & 30.2 & 45.5 & 14.8 & 4.6 & 1.2 & 0.3 \\
%  & \checkmark & $-$ & 20.7  & 34.9 & 7.2 & 1.0 & 0.3 & 0.1 \\
%  & $-$ & \checkmark & 31.9 & 46.9 & 16.9 & 5.8 & 2.0 & 0.5\\
%  \hline 
% \end{tabular} 
% \end{table} 


==> tables/SOTA_comparison.tex <==
\begin{table*}[t] 
\centering 
\tiny 
\caption{The AR are reported for the different classes,   methods and ranges.} 
 
\setlength{\tabcolsep}{2pt}\begin{tabular}{l|ccccccccccccccccccccccccccc} 
 
 % \hline \\
 %  Method & \rot{mAP } & \rot{Articulated Bus } & \rot{Bicycle } & \rot{Bicyclist } & \rot{Bollard } & \rot{Box Truck } & \rot{Bus } & \rot{C-Barrel } & \rot{C-Cone } & \rot{Dog } & \rot{Large Vehicle } & \rot{MBT } & \rot{MPC-Sign } & \rot{Motorcyle } & \rot{Motorcyclist } & \rot{Pedestrian } & \rot{Vehicle } & \rot{School Bus } & \rot{Sign } & \rot{Stop Sign } & \rot{Stroller } & \rot{Truck } & \rot{Truck Cab } & \rot{Trailer } & \rot{Wheelchair } & \rot{W-Device } & \rot{W-Rider }\\
 \hline \hline\\ 
  Method  & \rot{Average} & \rot{Vehicle } & \rot{Bus } & \rot{Pedestrian } & \rot{Stop Sign } & \rot{Box Truck } & \rot{Bollard } & \rot{C-Barrel } & \rot{Motorcyclist } & \rot{MPC-Sign } & \rot{Motorcycle } & \rot{Bicycle } & \rot{A-Bus } & \rot{School Bus } & \rot{Truck Cab } & \rot{C-Cone } & \rot{V-Trailer } & \rot{Sign } & \rot{Large Vehicle } & \rot{Stroller } & \rot{Bicyclist } & \rot{Truck } & \rot{MBT } & \rot{Dog } & \rot{Wheelchair } & \rot{W-Device } & \rot{W-Rider }\\
 \hline
 CenterPoint$\dagger$ & $13.5$& $61.0$& $36.0$& $33.0$& $28.0$& $26.0$& $25.0$& $22.5$& $16.0$& $16.0$& $12.5$& $9.5$& $8.5$& $7.5$& $8.0$& $8.0$& $7.0$& $6.5$& $3.0$& $2.0$& $14.0$& $14.0$& $1.0$& $0.5$& $0$& $3.0$& $0$ \\
 
 CenterPoint$\ddagger$ & $22.0$& $67.6$& $38.9$& $46.5$& $16.9$& $37.4$& $40.1$& $32.2$& $28.6$& $27.4$& $33.4$& $24.5$& $8.7$& $25.8$& $22.6$& $29.5$& $22.4$& $6.3$& $3.9$& $0.5$& $20.1$& $22.1$& $0$& $3.9$& $0.5$& $10.9$& $4.2$ \\
 
 FSD & $28.2$& $68.1$& $40.9$& $59.0$& $29.0$& $38.5$& $41.8$& $42.6$& $39.7$& $26.2$& $49.0$& $38.6$& $20.4$& $30.5$& $14.8$& $41.2$& $26.9$& $11.9$& $5.9$& $13.8$& $33.4$& $21.1$& $0$& $9.5$& $7.1$& $14.0$& $9.2$ \\

 VoxelNeXt & $30.7$& $72.7$& $38.8$& $63.2$& $40.2$& $40.1$& $53.9$& $64.9$& $44.7$& $39.4$& $42.4$& $40.6$& $20.1$& $25.2$& $19.9$& $44.9$& $20.9$& $14.9$& $6.8$& $15.7$& $32.4$& $16.9$& $0$& $14.4$& $0.1$& $17.4$& $6.6$\\
 
 FSF & $33.2$& $70.8$& $44.1$& $60.8$& $27.7$& $40.2$& $41.1$& $50.9$& $48.9$& $28.3$& $60.9$& $47.6$& $22.7$& $36.1$& $26.7$& $51.7$& $28.1$& $12.2$& $6.8$& $25.0.6$& $41.6$& $-$& $-$& $-$& $-$& $-$& $-$ \\
 
 FSD* & $29.8$& $71.5$& $40.5$& $66.4$& $31.2$& $37.2$& $51.5$& $52.7$& $43.2$& $25.8$& $51.5$& $41.6$& $18.8$& $30.4$& $19.9$& $45.5$& $27.5$& $12.1$& $5.6$& $15.1$& $35.4$& $20.0$& $0$& $2.1$& $1.9$& $17.4$& $9.1$ \\
 
 FSD$\_$Range & $31.9$& $74.5$& $42.1$& $69.2$& $32.0$& $39.1$& $53.3$& $58.7$& $50.1$& $27.4$& $55.9$& $46.1$& $21.2$& $30.5$& $20.2$& $54.8$& $26.4$& $12.0$& $6.2$& $15.9$& $42.6$& $21.4$& $0$& $1.9$& $2.3$& $17.2$& $9.5$ \\
 
 FSDv2 & $37.6$& $77.0$& $47.6$& $70.5$& $43.6$& $41.5$& $53.9$& $58.5$& $56.8$& $39.0$& $60.7$& $49.4$& $28.4$& $41.9$& $30.2$& $44.9$& $33.4$& $16.6$& $7.3$& $32.5$& $45.9$& $24.0$& $1.0$& $12.6$& $17.1$& $26.3$& $17.2$ \\
 
 FSDv2$\_$Range & $38.5$& $78.5$& $48.4$& $72.8$& $43.0$& $41.5$& $56.1$& $65.1$& $60.2$& $48.8$& $63.8$& $53.2$& $29.6$& $40.6$& $30.3$& $55.9$& $31.3$& $16.2$& $7.3$& $30.3$& $48.9$& $23.8$& $0$& $14.6$& $1.4$& $25.0$& $14.7$ \\
 \hline 
 \hline 
\end{tabular} 
\end{table*} 


==> tables/Tabulated_FSD+MVP_finetuned_pts_100.tex <==
\begin{table*}
\footnotesize 
 \caption{Results from FSD+MVP finetuned/pts 100.parquet}
\begin{tabular}{lrrrrrrrrrrrrrrrrrrrrrrrrrrr}
\toprule
 & \rot{Articulated Bus } & \rot{Bicycle } & \rot{Bicyclist } & \rot{Bollard } & \rot{Box Truck } & \rot{Bus } & \rot{Constr. Barrel } & \rot{Const. Cone } & \rot{Dog } & \rot{Large Vehicle } & \rot{Message Board Trailer } & \rot{M. Ped. Cross. Sign } & \rot{Motorcyle } & \rot{Motorcyclist } & \rot{Pedestrian } & \rot{Vehicle } & \rot{School Bus } & \rot{Sign } & \rot{Stop Sign } & \rot{Stroller } & \rot{Truck } & \rot{Truck Cab } & \rot{Trailer } & \rot{Wheelchair } & \rot{Wheeled Device } & \rot{Wheeled Rider } & \rot{Average Metrics } \\
\midrule
AP & 0.06 & 0.10 & 0.20 & 0.21 & 0.23 & 0.31 & 0.27 & 0.07 & 0.01 & 0.05 & 0.00 & 0.09 & 0.10 & 0.08 & 0.44 & 0.60 & 0.10 & 0.03 & 0.03 & 0.00 & 0.19 & 0.08 & 0.12 & 0.00 & 0.00 & 0.01 & 0.13 \\
ATE & 1.03 & 0.40 & 0.28 & 0.17 & 0.68 & 0.69 & 0.14 & 0.13 & 0.33 & 0.73 & 0.87 & 0.16 & 0.34 & 0.32 & 0.30 & 0.48 & 0.62 & 0.32 & 0.25 & 0.68 & 0.59 & 0.89 & 0.82 & 0.27 & 0.43 & 0.30 & 0.47 \\
ASE & 0.31 & 0.34 & 0.29 & 0.54 & 0.27 & 0.21 & 0.32 & 0.53 & 0.41 & 0.32 & 0.19 & 0.51 & 0.33 & 0.35 & 0.30 & 0.20 & 0.20 & 0.35 & 0.42 & 0.47 & 0.21 & 0.31 & 0.24 & 0.41 & 0.27 & 0.33 & 0.33 \\
AOE & 0.53 & 0.80 & 0.78 & 1.14 & 0.11 & 0.24 & 0.55 & 1.00 & 1.78 & 0.61 & 0.06 & 1.37 & 0.87 & 1.13 & 1.18 & 0.58 & 0.18 & 0.31 & 0.67 & 0.20 & 0.17 & 0.24 & 0.76 & 1.07 & 0.84 & 1.10 & 0.70 \\
CDS & 0.04 & 0.07 & 0.16 & 0.14 & 0.18 & 0.25 & 0.22 & 0.05 & 0.00 & 0.04 & 0.00 & 0.06 & 0.07 & 0.06 & 0.32 & 0.48 & 0.08 & 0.03 & 0.03 & 0.00 & 0.15 & 0.06 & 0.08 & 0.00 & 0.00 & 0.01 & 0.10 \\
\#GT & 558.00 & 4131.00 & 2018.00 & 23300.00 & 5214.00 & 3772.00 & 15093.00 & 7296.00 & 341.00 & 5079.00 & 64.00 & 448.00 & 1219.00 & 547.00 & 66309.00 & 245887.00 & 1061.00 & 4078.00 & 9056.00 & 175.00 & 2764.00 & 1831.00 & 2790.00 & 150.00 & 3051.00 & 666.00 & 15649.92 \\
\#Det & 6699.00 & 10555.00 & 12306.00 & 47000.00 & 11280.00 & 11331.00 & 21804.00 & 15670.00 & 1630.00 & 17939.00 & 1911.00 & 4860.00 & 8277.00 & 8602.00 & 150039.00 & 352584.00 & 4382.00 & 18275.00 & 23014.00 & 3679.00 & 11109.00 & 5071.00 & 8152.00 & 3944.00 & 4614.00 & 7500.00 & 29701.04 \\
\#TP & 103.50 & 937.00 & 904.00 & 9364.25 & 1960.00 & 1716.75 & 5834.25 & 1696.00 & 39.25 & 1100.00 & 6.75 & 93.75 & 384.25 & 303.50 & 39101.25 & 166425.50 & 235.00 & 931.75 & 1641.50 & 3.00 & 1177.75 & 349.25 & 600.00 & 9.00 & 169.50 & 59.00 & 9044.07 \\
AR & 0.18 & 0.23 & 0.45 & 0.40 & 0.38 & 0.46 & 0.39 & 0.23 & 0.12 & 0.22 & 0.10 & 0.21 & 0.32 & 0.56 & 0.59 & 0.68 & 0.22 & 0.23 & 0.18 & 0.02 & 0.43 & 0.19 & 0.21 & 0.06 & 0.06 & 0.09 & 0.28 \\
\bottomrule
\end{tabular}
\end{table*}


==> tables/Tabulated_FSD+MVP_finetuned_pts_150.tex <==
\begin{table*}
\footnotesize 
 \caption{Results from FSD+MVP finetuned/pts 150.parquet}
\begin{tabular}{lrrrrrrrrrrrrrrrrrrrrrrrrrrr}
\toprule
 & \rot{Articulated Bus } & \rot{Bicycle } & \rot{Bicyclist } & \rot{Bollard } & \rot{Box Truck } & \rot{Bus } & \rot{Constr. Barrel } & \rot{Const. Cone } & \rot{Dog } & \rot{Large Vehicle } & \rot{Message Board Trailer } & \rot{M. Ped. Cross. Sign } & \rot{Motorcyle } & \rot{Motorcyclist } & \rot{Pedestrian } & \rot{Vehicle } & \rot{School Bus } & \rot{Sign } & \rot{Stop Sign } & \rot{Stroller } & \rot{Truck } & \rot{Truck Cab } & \rot{Trailer } & \rot{Wheelchair } & \rot{Wheeled Device } & \rot{Wheeled Rider } & \rot{Average Metrics } \\
\midrule
AP & 0.02 & 0.01 & 0.01 & 0.03 & 0.09 & 0.17 & 0.06 & 0.03 & 0.00 & 0.02 & 0.00 & 0.00 & 0.02 & 0.01 & 0.19 & 0.37 & 0.00 & 0.00 & 0.00 & 0.00 & 0.04 & 0.02 & 0.03 & 0.00 & 0.00 & 0.00 & 0.04 \\
ATE & 0.59 & 0.43 & 0.42 & 0.23 & 0.99 & 0.81 & 0.20 & 0.18 & 2.00 & 0.99 & 2.00 & 0.17 & 0.47 & 0.34 & 0.40 & 0.65 & 1.10 & 0.40 & 0.40 & 1.84 & 0.82 & 1.01 & 0.85 & 2.00 & 0.40 & 0.36 & 0.77 \\
ASE & 0.15 & 0.33 & 0.31 & 0.55 & 0.33 & 0.23 & 0.51 & 0.62 & 1.00 & 0.37 & 1.00 & 0.66 & 0.38 & 0.42 & 0.38 & 0.25 & 0.27 & 0.42 & 0.40 & 0.52 & 0.25 & 0.29 & 0.20 & 1.00 & 0.32 & 0.27 & 0.44 \\
AOE & 0.06 & 1.44 & 1.32 & 1.34 & 0.22 & 0.27 & 0.99 & 2.17 & 3.14 & 0.43 & 3.14 & 1.97 & 1.02 & 1.77 & 1.40 & 0.90 & 0.25 & 0.14 & 1.36 & 1.03 & 0.26 & 0.12 & 1.58 & 3.14 & 1.65 & 0.03 & 1.20 \\
CDS & 0.02 & 0.01 & 0.01 & 0.02 & 0.07 & 0.13 & 0.04 & 0.01 & 0.00 & 0.02 & 0.00 & 0.00 & 0.01 & 0.01 & 0.12 & 0.27 & 0.00 & 0.00 & 0.00 & 0.00 & 0.03 & 0.01 & 0.02 & 0.00 & 0.00 & 0.00 & 0.03 \\
\#GT & 205.00 & 1251.00 & 934.00 & 3952.00 & 2316.00 & 2500.00 & 6630.00 & 2171.00 & 3.00 & 4045.00 & 0.00 & 114.00 & 498.00 & 347.00 & 20343.00 & 97700.00 & 574.00 & 1664.00 & 3259.00 & 12.00 & 1100.00 & 899.00 & 1223.00 & 48.00 & 669.00 & 154.00 & 5869.65 \\
\#Det & 1200.00 & 1465.00 & 2944.00 & 4172.00 & 7295.00 & 6647.00 & 7792.00 & 753.00 & 0.00 & 11243.00 & 0.00 & 3541.00 & 799.00 & 957.00 & 52272.00 & 202036.00 & 1899.00 & 6251.00 & 7953.00 & 435.00 & 5937.00 & 2337.00 & 2387.00 & 19.00 & 128.00 & 267.00 & 12720.35 \\
\#TP & 25.00 & 103.00 & 119.75 & 434.25 & 544.50 & 771.00 & 1180.25 & 154.50 & 0.00 & 734.25 & 0.00 & 14.00 & 54.75 & 48.50 & 7511.75 & 50104.00 & 33.75 & 139.50 & 151.00 & 0.50 & 279.75 & 96.75 & 99.25 & 0.00 & 1.75 & 1.00 & 2407.80 \\
AR & 0.12 & 0.08 & 0.13 & 0.11 & 0.23 & 0.31 & 0.18 & 0.07 & 0.00 & 0.18 & 0.00 & 0.12 & 0.11 & 0.14 & 0.37 & 0.51 & 0.06 & 0.08 & 0.05 & 0.04 & 0.25 & 0.11 & 0.08 & 0.00 & 0.00 & 0.01 & 0.13 \\
\bottomrule
\end{tabular}
\end{table*}


==> tables/Tabulated_FSD+MVP_finetuned_pts_200.tex <==
\begin{table*}
\footnotesize 
 \caption{Results from FSD+MVP finetuned/pts 200.parquet}
\begin{tabular}{lrrrrrrrrrrrrrrrrrrrrrrrrrrr}
\toprule
 & \rot{Articulated Bus } & \rot{Bicycle } & \rot{Bicyclist } & \rot{Bollard } & \rot{Box Truck } & \rot{Bus } & \rot{Constr. Barrel } & \rot{Const. Cone } & \rot{Dog } & \rot{Large Vehicle } & \rot{Message Board Trailer } & \rot{M. Ped. Cross. Sign } & \rot{Motorcyle } & \rot{Motorcyclist } & \rot{Pedestrian } & \rot{Vehicle } & \rot{School Bus } & \rot{Sign } & \rot{Stop Sign } & \rot{Stroller } & \rot{Truck } & \rot{Truck Cab } & \rot{Trailer } & \rot{Wheelchair } & \rot{Wheeled Device } & \rot{Wheeled Rider } & \rot{Average Metrics } \\
\midrule
AP & 0.00 & 0.00 & 0.00 & 0.01 & 0.05 & 0.03 & 0.02 & 0.00 & 0.00 & 0.04 & 0.00 & 0.00 & 0.00 & 0.00 & 0.05 & 0.22 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.01 & 0.01 & 0.00 & 0.00 & 0.00 & 0.02 \\
ATE & 0.94 & 0.55 & 0.66 & 0.42 & 1.11 & 1.02 & 0.27 & 2.00 & 2.00 & 1.03 & 2.00 & 2.00 & 2.00 & 2.00 & 0.49 & 0.72 & 0.99 & 0.53 & 0.35 & 2.00 & 0.66 & 1.09 & 0.80 & 2.00 & 2.00 & 2.00 & 1.22 \\
ASE & 0.20 & 0.51 & 0.24 & 0.79 & 0.36 & 0.34 & 0.53 & 1.00 & 1.00 & 0.34 & 1.00 & 1.00 & 1.00 & 1.00 & 0.43 & 0.28 & 0.36 & 0.42 & 0.40 & 1.00 & 0.27 & 0.28 & 0.18 & 1.00 & 1.00 & 1.00 & 0.61 \\
AOE & 0.01 & 0.32 & 1.36 & 1.31 & 0.36 & 0.56 & 1.19 & 3.14 & 3.14 & 0.32 & 3.14 & 3.14 & 3.14 & 3.14 & 1.68 & 1.03 & 0.03 & 0.05 & 0.14 & 3.14 & 0.73 & 0.26 & 1.31 & 3.14 & 3.14 & 3.14 & 1.62 \\
CDS & 0.00 & 0.00 & 0.00 & 0.00 & 0.03 & 0.02 & 0.01 & 0.00 & 0.00 & 0.03 & 0.00 & 0.00 & 0.00 & 0.00 & 0.03 & 0.15 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.01 & 0.01 & 0.00 & 0.00 & 0.00 & 0.01 \\
\#GT & 64.00 & 143.00 & 192.00 & 910.00 & 1356.00 & 1476.00 & 2355.00 & 81.00 & 0.00 & 2637.00 & 0.00 & 15.00 & 25.00 & 18.00 & 3100.00 & 25305.00 & 287.00 & 670.00 & 1014.00 & 0.00 & 296.00 & 466.00 & 666.00 & 0.00 & 30.00 & 9.00 & 1581.35 \\
\#Det & 889.00 & 37.00 & 117.00 & 10.00 & 3191.00 & 3366.00 & 327.00 & 0.00 & 0.00 & 4990.00 & 0.00 & 530.00 & 18.00 & 18.00 & 3099.00 & 55369.00 & 491.00 & 1222.00 & 1840.00 & 0.00 & 1620.00 & 1296.00 & 513.00 & 0.00 & 29.00 & 0.00 & 3037.39 \\
\#TP & 2.50 & 0.75 & 2.50 & 3.00 & 218.75 & 199.50 & 96.25 & 0.00 & 0.00 & 436.00 & 0.00 & 0.00 & 0.00 & 0.00 & 452.25 & 9883.50 & 3.50 & 26.25 & 27.25 & 0.00 & 30.50 & 52.50 & 36.75 & 0.00 & 0.00 & 0.00 & 441.22 \\
AR & 0.04 & 0.01 & 0.01 & 0.00 & 0.16 & 0.14 & 0.04 & 0.00 & 0.00 & 0.17 & 0.00 & 0.00 & 0.00 & 0.00 & 0.15 & 0.39 & 0.01 & 0.04 & 0.03 & 0.00 & 0.10 & 0.11 & 0.06 & 0.00 & 0.00 & 0.00 & 0.06 \\
\bottomrule
\end{tabular}
\end{table*}


==> tables/Tabulated_FSD+MVP_finetuned_pts_250.tex <==
\begin{table*}
\footnotesize 
 \caption{Results from FSD+MVP finetuned/pts 250.parquet}
\begin{tabular}{lrrrrrrrrrrrrrrrrrrrrrrrrrrr}
\toprule
 & \rot{Articulated Bus } & \rot{Bicycle } & \rot{Bicyclist } & \rot{Bollard } & \rot{Box Truck } & \rot{Bus } & \rot{Constr. Barrel } & \rot{Const. Cone } & \rot{Dog } & \rot{Large Vehicle } & \rot{Message Board Trailer } & \rot{M. Ped. Cross. Sign } & \rot{Motorcyle } & \rot{Motorcyclist } & \rot{Pedestrian } & \rot{Vehicle } & \rot{School Bus } & \rot{Sign } & \rot{Stop Sign } & \rot{Stroller } & \rot{Truck } & \rot{Truck Cab } & \rot{Trailer } & \rot{Wheelchair } & \rot{Wheeled Device } & \rot{Wheeled Rider } & \rot{Average Metrics } \\
\midrule
AP & 0.00 & 0.00 & 0.00 & 0.00 & 0.04 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.07 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 \\
ATE & 2.00 & 2.00 & 2.00 & 2.00 & 0.84 & 1.91 & 2.00 & 2.00 & 2.00 & 1.40 & 2.00 & 2.00 & 2.00 & 2.00 & 2.00 & 0.81 & 2.00 & 0.24 & 2.00 & 2.00 & 0.61 & 0.82 & 2.00 & 2.00 & 2.00 & 2.00 & 1.72 \\
ASE & 1.00 & 1.00 & 1.00 & 1.00 & 0.30 & 0.50 & 1.00 & 1.00 & 1.00 & 0.42 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 0.30 & 1.00 & 0.43 & 1.00 & 1.00 & 0.17 & 0.18 & 1.00 & 1.00 & 1.00 & 1.00 & 0.82 \\
AOE & 3.14 & 3.14 & 3.14 & 3.14 & 0.06 & 3.05 & 3.14 & 3.14 & 3.14 & 0.46 & 3.14 & 3.14 & 3.14 & 3.14 & 3.14 & 0.94 & 3.14 & 0.02 & 3.14 & 3.14 & 3.11 & 0.03 & 3.14 & 3.14 & 3.14 & 3.14 & 2.59 \\
CDS & 0.00 & 0.00 & 0.00 & 0.00 & 0.03 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.04 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
\#GT & 1.00 & 0.00 & 0.00 & 61.00 & 242.00 & 66.00 & 340.00 & 0.00 & 0.00 & 399.00 & 0.00 & 0.00 & 0.00 & 0.00 & 149.00 & 2705.00 & 110.00 & 49.00 & 38.00 & 0.00 & 39.00 & 112.00 & 129.00 & 0.00 & 0.00 & 0.00 & 170.77 \\
\#Det & 45.00 & 0.00 & 0.00 & 0.00 & 227.00 & 216.00 & 0.00 & 0.00 & 0.00 & 310.00 & 0.00 & 0.00 & 0.00 & 0.00 & 16.00 & 2838.00 & 17.00 & 7.00 & 15.00 & 0.00 & 54.00 & 72.00 & 5.00 & 0.00 & 0.00 & 0.00 & 147.00 \\
\#TP & 0.00 & 0.00 & 0.00 & 0.00 & 14.50 & 1.25 & 0.00 & 0.00 & 0.00 & 19.25 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 424.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.75 & 8.00 & 0.50 & 0.00 & 0.00 & 0.00 & 18.09 \\
AR & 0.00 & 0.00 & 0.00 & 0.00 & 0.06 & 0.02 & 0.00 & 0.00 & 0.00 & 0.05 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.16 & 0.00 & 0.02 & 0.00 & 0.00 & 0.04 & 0.07 & 0.00 & 0.00 & 0.00 & 0.00 & 0.02 \\
\bottomrule
\end{tabular}
\end{table*}


==> tables/Tabulated_FSD+MVP_finetuned_pts_50.tex <==
\begin{table*}
\footnotesize 
 \caption{Results from FSD+MVP finetuned/pts 50.parquet}
\begin{tabular}{lrrrrrrrrrrrrrrrrrrrrrrrrrrr}
\toprule
 & \rot{Articulated Bus } & \rot{Bicycle } & \rot{Bicyclist } & \rot{Bollard } & \rot{Box Truck } & \rot{Bus } & \rot{Constr. Barrel } & \rot{Const. Cone } & \rot{Dog } & \rot{Large Vehicle } & \rot{Message Board Trailer } & \rot{M. Ped. Cross. Sign } & \rot{Motorcyle } & \rot{Motorcyclist } & \rot{Pedestrian } & \rot{Vehicle } & \rot{School Bus } & \rot{Sign } & \rot{Stop Sign } & \rot{Stroller } & \rot{Truck } & \rot{Truck Cab } & \rot{Trailer } & \rot{Wheelchair } & \rot{Wheeled Device } & \rot{Wheeled Rider } & \rot{Average Metrics } \\
\midrule
AP & 0.30 & 0.51 & 0.61 & 0.64 & 0.65 & 0.68 & 0.76 & 0.58 & 0.03 & 0.10 & 0.00 & 0.51 & 0.64 & 0.60 & 0.82 & 0.89 & 0.70 & 0.19 & 0.51 & 0.13 & 0.30 & 0.29 & 0.43 & 0.01 & 0.21 & 0.14 & 0.43 \\
ATE & 0.80 & 0.28 & 0.22 & 0.08 & 0.44 & 0.42 & 0.09 & 0.09 & 0.35 & 0.60 & 2.00 & 0.06 & 0.20 & 0.24 & 0.19 & 0.28 & 0.43 & 0.25 & 0.14 & 0.22 & 0.51 & 0.75 & 0.64 & 0.18 & 0.31 & 0.34 & 0.39 \\
ASE & 0.15 & 0.23 & 0.24 & 0.44 & 0.19 & 0.15 & 0.23 & 0.43 & 0.47 & 0.28 & 1.00 & 0.38 & 0.23 & 0.30 & 0.21 & 0.14 & 0.12 & 0.31 & 0.39 & 0.31 & 0.16 & 0.26 & 0.17 & 0.32 & 0.16 & 0.34 & 0.29 \\
AOE & 0.24 & 0.50 & 0.22 & 0.86 & 0.08 & 0.06 & 0.91 & 0.89 & 1.10 & 0.50 & 3.14 & 1.39 & 0.34 & 0.29 & 0.70 & 0.17 & 0.04 & 0.51 & 0.29 & 0.32 & 0.08 & 0.16 & 0.49 & 1.21 & 0.61 & 0.70 & 0.61 \\
CDS & 0.23 & 0.42 & 0.53 & 0.48 & 0.55 & 0.59 & 0.62 & 0.44 & 0.02 & 0.08 & 0.00 & 0.37 & 0.55 & 0.49 & 0.67 & 0.79 & 0.62 & 0.15 & 0.41 & 0.10 & 0.26 & 0.23 & 0.33 & 0.01 & 0.17 & 0.10 & 0.35 \\
\#GT & 755.00 & 13864.00 & 2480.00 & 55604.00 & 6543.00 & 5094.00 & 24962.00 & 24555.00 & 1375.00 & 5844.00 & 4.00 & 434.00 & 4592.00 & 1365.00 & 150560.00 & 375089.00 & 1095.00 & 7294.00 & 16362.00 & 635.00 & 4193.00 & 3517.00 & 5478.00 & 426.00 & 10074.00 & 1616.00 & 27838.85 \\
\#Det & 3287.00 & 45737.00 & 11420.00 & 103613.00 & 10648.00 & 8484.00 & 42115.00 & 53282.00 & 24394.00 & 16741.00 & 606.00 & 3786.00 & 18289.00 & 6648.00 & 227785.00 & 423528.00 & 2481.00 & 33615.00 & 50962.00 & 15444.00 & 9994.00 & 5043.00 & 12418.00 & 10098.00 & 30941.00 & 8320.00 & 45372.27 \\
\#TP & 307.50 & 8951.25 & 1851.75 & 41234.00 & 4855.25 & 3800.25 & 20155.75 & 16772.50 & 472.00 & 2145.75 & 0.00 & 307.00 & 3467.25 & 1106.25 & 129210.75 & 342803.50 & 860.00 & 3347.50 & 10675.75 & 348.50 & 2331.50 & 1309.00 & 2798.75 & 115.25 & 3959.50 & 507.00 & 23218.98 \\
AR & 0.41 & 0.65 & 0.75 & 0.74 & 0.74 & 0.75 & 0.81 & 0.68 & 0.34 & 0.37 & 0.00 & 0.71 & 0.76 & 0.81 & 0.86 & 0.91 & 0.79 & 0.46 & 0.65 & 0.55 & 0.56 & 0.37 & 0.51 & 0.27 & 0.39 & 0.31 & 0.58 \\
\bottomrule
\end{tabular}
\end{table*}


==> tables/Tabulated_ImFSD_minpts=1_combined_0-250.tex <==
\begin{table*}
\footnotesize 
 \caption{Results from ImFSD minpts=1/combined 0-250.parquet}
\begin{tabular}{lrrrrrrrrrrrrrrrrrrrrrrrrrrr}
\toprule
 & \rot{Articulated Bus } & \rot{Bicycle } & \rot{Bicyclist } & \rot{Bollard } & \rot{Box Truck } & \rot{Bus } & \rot{Constr. Barrel } & \rot{Const. Cone } & \rot{Dog } & \rot{Large Vehicle } & \rot{Message Board Trailer } & \rot{M. Ped. Cross. Sign } & \rot{Motorcyle } & \rot{Motorcyclist } & \rot{Pedestrian } & \rot{Vehicle } & \rot{School Bus } & \rot{Sign } & \rot{Stop Sign } & \rot{Stroller } & \rot{Truck } & \rot{Truck Cab } & \rot{Trailer } & \rot{Wheelchair } & \rot{Wheeled Device } & \rot{Wheeled Rider } & \rot{Average Metrics } \\
\midrule
AP & 0.19 & 0.38 & 0.33 & 0.47 & 0.36 & 0.39 & 0.44 & 0.43 & 0.10 & 0.05 & 0.00 & 0.25 & 0.48 & 0.39 & 0.63 & 0.70 & 0.29 & 0.11 & 0.29 & 0.13 & 0.20 & 0.18 & 0.25 & 0.07 & 0.14 & 0.09 & 0.28 \\
ATE & 0.77 & 0.29 & 0.25 & 0.10 & 0.57 & 0.55 & 0.10 & 0.09 & 0.38 & 0.71 & 2.00 & 0.09 & 0.23 & 0.27 & 0.22 & 0.39 & 0.54 & 0.28 & 0.16 & 0.21 & 0.57 & 0.84 & 0.72 & 0.16 & 0.30 & 0.32 & 0.43 \\
ASE & 0.20 & 0.24 & 0.26 & 0.47 & 0.23 & 0.18 & 0.26 & 0.43 & 0.45 & 0.31 & 1.00 & 0.44 & 0.25 & 0.31 & 0.24 & 0.17 & 0.15 & 0.32 & 0.40 & 0.31 & 0.18 & 0.29 & 0.19 & 0.32 & 0.16 & 0.34 & 0.31 \\
AOE & 0.35 & 0.50 & 0.45 & 0.94 & 0.10 & 0.16 & 0.88 & 0.91 & 0.95 & 0.43 & 3.14 & 1.54 & 0.37 & 0.52 & 0.84 & 0.40 & 0.09 & 0.51 & 0.36 & 0.29 & 0.14 & 0.26 & 0.62 & 1.56 & 0.58 & 0.78 & 0.68 \\
CDS & 0.15 & 0.31 & 0.27 & 0.34 & 0.29 & 0.33 & 0.35 & 0.32 & 0.07 & 0.04 & 0.00 & 0.17 & 0.41 & 0.31 & 0.50 & 0.58 & 0.25 & 0.08 & 0.23 & 0.11 & 0.17 & 0.13 & 0.19 & 0.05 & 0.12 & 0.07 & 0.22 \\
\#GT & 1583.00 & 19389.00 & 5624.00 & 83827.00 & 15671.00 & 12908.00 & 49380.00 & 34103.00 & 1719.00 & 18004.00 & 68.00 & 1011.00 & 6334.00 & 2277.00 & 240461.00 & 746686.00 & 3127.00 & 13755.00 & 29729.00 & 822.00 & 8392.00 & 6825.00 & 10286.00 & 624.00 & 13824.00 & 2445.00 & 51110.54 \\
\#Det & 15316.00 & 68632.00 & 38737.00 & 172253.00 & 47678.00 & 42283.00 & 76429.00 & 80387.00 & 3286.00 & 60900.00 & 337.00 & 23313.00 & 36714.00 & 28919.00 & 487036.00 & 1134445.00 & 14607.00 & 77893.00 & 110136.00 & 27594.00 & 37248.00 & 20543.00 & 29960.00 & 687.00 & 42283.00 & 28522.00 & 104082.23 \\
\#TP & 518.50 & 9687.00 & 2740.00 & 49640.25 & 7423.75 & 6429.25 & 25271.00 & 18319.00 & 501.25 & 3738.25 & 0.00 & 438.75 & 3856.00 & 1448.75 & 169714.25 & 557392.50 & 1196.00 & 4163.75 & 12025.00 & 338.75 & 3744.50 & 1952.50 & 3491.00 & 127.00 & 4000.50 & 581.00 & 34182.25 \\
AR & 0.33 & 0.50 & 0.49 & 0.59 & 0.47 & 0.50 & 0.51 & 0.54 & 0.29 & 0.21 & 0.00 & 0.43 & 0.61 & 0.64 & 0.71 & 0.75 & 0.38 & 0.30 & 0.40 & 0.41 & 0.45 & 0.29 & 0.34 & 0.20 & 0.29 & 0.24 & 0.42 \\
\bottomrule
\end{tabular}
\end{table*}


==> tables/Tabulated_ImFSD_minpts=1_combined_100.tex <==
\begin{table*}
\footnotesize 
 \caption{Results from ImFSD minpts=1/combined 100.parquet}
\begin{tabular}{lrrrrrrrrrrrrrrrrrrrrrrrrrrr}
\toprule
 & \rot{Articulated Bus } & \rot{Bicycle } & \rot{Bicyclist } & \rot{Bollard } & \rot{Box Truck } & \rot{Bus } & \rot{Constr. Barrel } & \rot{Const. Cone } & \rot{Dog } & \rot{Large Vehicle } & \rot{Message Board Trailer } & \rot{M. Ped. Cross. Sign } & \rot{Motorcyle } & \rot{Motorcyclist } & \rot{Pedestrian } & \rot{Vehicle } & \rot{School Bus } & \rot{Sign } & \rot{Stop Sign } & \rot{Stroller } & \rot{Truck } & \rot{Truck Cab } & \rot{Trailer } & \rot{Wheelchair } & \rot{Wheeled Device } & \rot{Wheeled Rider } & \rot{Average Metrics } \\
\midrule
AP & 0.05 & 0.09 & 0.19 & 0.16 & 0.22 & 0.30 & 0.19 & 0.07 & 0.03 & 0.05 & 0.00 & 0.10 & 0.10 & 0.08 & 0.40 & 0.59 & 0.09 & 0.04 & 0.03 & 0.00 & 0.18 & 0.12 & 0.12 & 0.02 & 0.00 & 0.01 & 0.12 \\
ATE & 1.00 & 0.40 & 0.28 & 0.18 & 0.67 & 0.69 & 0.14 & 0.13 & 0.27 & 0.75 & 2.00 & 0.14 & 0.36 & 0.33 & 0.30 & 0.50 & 0.65 & 0.34 & 0.24 & 0.54 & 0.64 & 0.84 & 0.83 & 0.10 & 0.44 & 0.34 & 0.50 \\
ASE & 0.33 & 0.34 & 0.28 & 0.55 & 0.27 & 0.22 & 0.34 & 0.54 & 0.45 & 0.32 & 1.00 & 0.50 & 0.33 & 0.37 & 0.31 & 0.20 & 0.20 & 0.35 & 0.43 & 0.60 & 0.21 & 0.30 & 0.24 & 0.56 & 0.30 & 0.34 & 0.38 \\
AOE & 0.59 & 0.84 & 0.81 & 1.20 & 0.11 & 0.26 & 0.58 & 1.03 & 1.60 & 0.55 & 3.14 & 1.59 & 0.93 & 1.10 & 1.22 & 0.63 & 0.12 & 0.40 & 0.77 & 1.13 & 0.23 & 0.17 & 0.81 & 1.51 & 0.91 & 0.84 & 0.89 \\
CDS & 0.04 & 0.07 & 0.15 & 0.11 & 0.17 & 0.23 & 0.15 & 0.05 & 0.02 & 0.04 & 0.00 & 0.07 & 0.07 & 0.05 & 0.29 & 0.47 & 0.07 & 0.03 & 0.03 & 0.00 & 0.14 & 0.09 & 0.09 & 0.01 & 0.00 & 0.01 & 0.09 \\
\#GT & 558.00 & 4131.00 & 2018.00 & 23300.00 & 5214.00 & 3772.00 & 15093.00 & 7296.00 & 341.00 & 5079.00 & 64.00 & 448.00 & 1219.00 & 547.00 & 66309.00 & 245887.00 & 1061.00 & 4078.00 & 9056.00 & 175.00 & 2764.00 & 1831.00 & 2790.00 & 150.00 & 3051.00 & 666.00 & 15649.92 \\
\#Det & 7123.00 & 12769.00 & 18466.00 & 51895.00 & 16934.00 & 13668.00 & 24276.00 & 16155.00 & 196.00 & 21816.00 & 2.00 & 7375.00 & 12395.00 & 15458.00 & 181426.00 & 383293.00 & 6230.00 & 21189.00 & 26746.00 & 5231.00 & 15551.00 & 7112.00 & 10400.00 & 34.00 & 3932.00 & 13563.00 & 34355.19 \\
\#TP & 119.50 & 914.25 & 902.75 & 8524.75 & 2002.75 & 1748.25 & 4983.50 & 1614.50 & 24.50 & 1150.00 & 0.00 & 102.00 & 422.50 & 318.50 & 38065.25 & 165378.50 & 281.50 & 942.00 & 1591.25 & 2.75 & 1288.00 & 454.50 & 664.50 & 3.00 & 124.50 & 86.00 & 8911.90 \\
AR & 0.21 & 0.22 & 0.45 & 0.37 & 0.38 & 0.46 & 0.33 & 0.22 & 0.07 & 0.23 & 0.00 & 0.23 & 0.35 & 0.58 & 0.57 & 0.67 & 0.27 & 0.23 & 0.18 & 0.02 & 0.47 & 0.25 & 0.24 & 0.02 & 0.04 & 0.13 & 0.28 \\
\bottomrule
\end{tabular}
\end{table*}


==> tables/Tabulated_ImFSD_minpts=1_combined_150.tex <==
\begin{table*}
\footnotesize 
 \caption{Results from ImFSD minpts=1/combined 150.parquet}
\begin{tabular}{lrrrrrrrrrrrrrrrrrrrrrrrrrrr}
\toprule
 & \rot{Articulated Bus } & \rot{Bicycle } & \rot{Bicyclist } & \rot{Bollard } & \rot{Box Truck } & \rot{Bus } & \rot{Constr. Barrel } & \rot{Const. Cone } & \rot{Dog } & \rot{Large Vehicle } & \rot{Message Board Trailer } & \rot{M. Ped. Cross. Sign } & \rot{Motorcyle } & \rot{Motorcyclist } & \rot{Pedestrian } & \rot{Vehicle } & \rot{School Bus } & \rot{Sign } & \rot{Stop Sign } & \rot{Stroller } & \rot{Truck } & \rot{Truck Cab } & \rot{Trailer } & \rot{Wheelchair } & \rot{Wheeled Device } & \rot{Wheeled Rider } & \rot{Average Metrics } \\
\midrule
AP & 0.04 & 0.00 & 0.01 & 0.01 & 0.07 & 0.12 & 0.02 & 0.00 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.08 & 0.23 & 0.01 & 0.00 & 0.00 & 0.00 & 0.05 & 0.04 & 0.03 & 0.00 & 0.00 & 0.00 & 0.03 \\
ATE & 0.52 & 0.52 & 0.41 & 0.29 & 0.95 & 0.81 & 0.23 & 0.18 & 2.00 & 0.95 & 2.00 & 0.27 & 0.53 & 0.38 & 0.43 & 0.68 & 1.05 & 0.51 & 0.48 & 2.00 & 0.74 & 0.98 & 0.73 & 2.00 & 0.47 & 0.29 & 0.79 \\
ASE & 0.14 & 0.37 & 0.34 & 0.56 & 0.34 & 0.22 & 0.57 & 0.53 & 1.00 & 0.37 & 1.00 & 0.66 & 0.43 & 0.48 & 0.38 & 0.26 & 0.29 & 0.47 & 0.42 & 1.00 & 0.24 & 0.26 & 0.21 & 1.00 & 0.29 & 0.43 & 0.47 \\
AOE & 0.12 & 1.43 & 1.65 & 1.34 & 0.23 & 0.31 & 1.14 & 1.54 & 3.14 & 0.44 & 3.14 & 2.89 & 2.09 & 2.68 & 1.39 & 0.94 & 0.29 & 0.17 & 1.00 & 3.14 & 0.26 & 0.25 & 1.21 & 3.14 & 0.14 & 3.02 & 1.43 \\
CDS & 0.03 & 0.00 & 0.01 & 0.01 & 0.05 & 0.09 & 0.01 & 0.00 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.05 & 0.16 & 0.01 & 0.00 & 0.00 & 0.00 & 0.04 & 0.03 & 0.02 & 0.00 & 0.00 & 0.00 & 0.02 \\
\#GT & 205.00 & 1251.00 & 934.00 & 3952.00 & 2316.00 & 2500.00 & 6630.00 & 2171.00 & 3.00 & 4045.00 & 0.00 & 114.00 & 498.00 & 347.00 & 20343.00 & 97700.00 & 574.00 & 1664.00 & 3259.00 & 12.00 & 1100.00 & 899.00 & 1223.00 & 48.00 & 669.00 & 154.00 & 5869.65 \\
\#Det & 1719.00 & 926.00 & 3501.00 & 3809.00 & 10825.00 & 9576.00 & 3142.00 & 104.00 & 0.00 & 10639.00 & 0.00 & 8900.00 & 1350.00 & 2366.00 & 45871.00 & 229091.00 & 3562.00 & 11830.00 & 20561.00 & 788.00 & 6465.00 & 3905.00 & 3291.00 & 0.00 & 82.00 & 871.00 & 14737.46 \\
\#TP & 41.25 & 45.75 & 89.00 & 293.75 & 540.25 & 736.00 & 383.75 & 6.00 & 0.00 & 500.00 & 0.00 & 22.00 & 19.50 & 23.75 & 5231.50 & 41019.50 & 46.00 & 203.75 & 278.75 & 0.00 & 246.75 & 117.50 & 112.75 & 0.00 & 4.50 & 1.00 & 1921.65 \\
AR & 0.20 & 0.04 & 0.10 & 0.07 & 0.23 & 0.29 & 0.06 & 0.00 & 0.00 & 0.12 & 0.00 & 0.19 & 0.04 & 0.07 & 0.26 & 0.42 & 0.08 & 0.12 & 0.09 & 0.00 & 0.22 & 0.13 & 0.09 & 0.00 & 0.01 & 0.01 & 0.11 \\
\bottomrule
\end{tabular}
\end{table*}


==> tables/Tabulated_ImFSD_minpts=1_combined_200.tex <==
\begin{table*}
\footnotesize 
 \caption{Results from ImFSD minpts=1/combined 200.parquet}
\begin{tabular}{lrrrrrrrrrrrrrrrrrrrrrrrrrrr}
\toprule
 & \rot{Articulated Bus } & \rot{Bicycle } & \rot{Bicyclist } & \rot{Bollard } & \rot{Box Truck } & \rot{Bus } & \rot{Constr. Barrel } & \rot{Const. Cone } & \rot{Dog } & \rot{Large Vehicle } & \rot{Message Board Trailer } & \rot{M. Ped. Cross. Sign } & \rot{Motorcyle } & \rot{Motorcyclist } & \rot{Pedestrian } & \rot{Vehicle } & \rot{School Bus } & \rot{Sign } & \rot{Stop Sign } & \rot{Stroller } & \rot{Truck } & \rot{Truck Cab } & \rot{Trailer } & \rot{Wheelchair } & \rot{Wheeled Device } & \rot{Wheeled Rider } & \rot{Average Metrics } \\
\midrule
AP & 0.00 & 0.00 & 0.00 & 0.02 & 0.02 & 0.01 & 0.01 & 0.00 & 0.00 & 0.02 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.10 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.04 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 \\
ATE & 0.71 & 2.00 & 0.69 & 0.59 & 1.14 & 1.02 & 0.40 & 2.00 & 2.00 & 1.16 & 2.00 & 2.00 & 2.00 & 2.00 & 0.61 & 0.77 & 0.88 & 0.67 & 0.66 & 2.00 & 0.68 & 1.09 & 0.78 & 2.00 & 2.00 & 2.00 & 1.30 \\
ASE & 0.22 & 1.00 & 0.28 & 0.73 & 0.41 & 0.32 & 0.46 & 1.00 & 1.00 & 0.39 & 1.00 & 1.00 & 1.00 & 1.00 & 0.42 & 0.29 & 0.23 & 0.44 & 0.37 & 1.00 & 0.27 & 0.26 & 0.39 & 1.00 & 1.00 & 1.00 & 0.63 \\
AOE & 0.32 & 3.14 & 0.04 & 0.64 & 0.48 & 0.58 & 0.54 & 3.14 & 3.14 & 0.29 & 3.14 & 3.14 & 3.14 & 3.14 & 1.76 & 1.05 & 0.06 & 0.12 & 0.49 & 3.14 & 0.42 & 0.24 & 0.19 & 3.14 & 3.14 & 3.14 & 1.61 \\
CDS & 0.00 & 0.00 & 0.00 & 0.01 & 0.01 & 0.01 & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.06 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.03 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 \\
\#GT & 64.00 & 143.00 & 192.00 & 910.00 & 1356.00 & 1476.00 & 2355.00 & 81.00 & 0.00 & 2637.00 & 0.00 & 15.00 & 25.00 & 18.00 & 3100.00 & 25305.00 & 287.00 & 670.00 & 1014.00 & 0.00 & 296.00 & 466.00 & 666.00 & 0.00 & 30.00 & 9.00 & 1581.35 \\
\#Det & 1622.00 & 22.00 & 115.00 & 195.00 & 5425.00 & 7165.00 & 27.00 & 0.00 & 0.00 & 5387.00 & 0.00 & 2238.00 & 8.00 & 15.00 & 4373.00 & 105795.00 & 1205.00 & 3131.00 & 6701.00 & 0.00 & 1145.00 & 2241.00 & 574.00 & 0.00 & 2.00 & 0.00 & 5668.69 \\
\#TP & 9.00 & 0.00 & 1.75 & 33.25 & 184.00 & 128.75 & 3.00 & 0.00 & 0.00 & 275.75 & 0.00 & 0.00 & 0.00 & 0.00 & 221.00 & 8251.00 & 8.75 & 26.50 & 61.00 & 0.00 & 25.00 & 51.25 & 16.50 & 0.00 & 0.00 & 0.00 & 357.56 \\
AR & 0.14 & 0.00 & 0.01 & 0.04 & 0.14 & 0.09 & 0.00 & 0.00 & 0.00 & 0.10 & 0.00 & 0.00 & 0.00 & 0.00 & 0.07 & 0.33 & 0.03 & 0.04 & 0.06 & 0.00 & 0.08 & 0.11 & 0.03 & 0.00 & 0.00 & 0.00 & 0.05 \\
\bottomrule
\end{tabular}
\end{table*}


==> tables/Tabulated_ImFSD_minpts=1_combined_250.tex <==
\begin{table*}
\footnotesize 
 \caption{Results from ImFSD minpts=1/combined 250.parquet}
\begin{tabular}{lrrrrrrrrrrrrrrrrrrrrrrrrrrr}
\toprule
 & \rot{Articulated Bus } & \rot{Bicycle } & \rot{Bicyclist } & \rot{Bollard } & \rot{Box Truck } & \rot{Bus } & \rot{Constr. Barrel } & \rot{Const. Cone } & \rot{Dog } & \rot{Large Vehicle } & \rot{Message Board Trailer } & \rot{M. Ped. Cross. Sign } & \rot{Motorcyle } & \rot{Motorcyclist } & \rot{Pedestrian } & \rot{Vehicle } & \rot{School Bus } & \rot{Sign } & \rot{Stop Sign } & \rot{Stroller } & \rot{Truck } & \rot{Truck Cab } & \rot{Trailer } & \rot{Wheelchair } & \rot{Wheeled Device } & \rot{Wheeled Rider } & \rot{Average Metrics } \\
\midrule
AP & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.03 & 0.00 & 0.00 & 0.00 & 0.00 & 0.03 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
ATE & 2.00 & 2.00 & 2.00 & 2.00 & 1.28 & 2.00 & 2.00 & 2.00 & 2.00 & 1.37 & 2.00 & 2.00 & 2.00 & 2.00 & 1.46 & 0.83 & 2.00 & 2.00 & 0.93 & 2.00 & 1.06 & 0.94 & 2.00 & 2.00 & 2.00 & 2.00 & 1.76 \\
ASE & 1.00 & 1.00 & 1.00 & 1.00 & 0.44 & 1.00 & 1.00 & 1.00 & 1.00 & 0.36 & 1.00 & 1.00 & 1.00 & 1.00 & 0.33 & 0.31 & 1.00 & 1.00 & 0.18 & 1.00 & 0.18 & 0.32 & 1.00 & 1.00 & 1.00 & 1.00 & 0.81 \\
AOE & 3.14 & 3.14 & 3.14 & 3.14 & 0.36 & 3.14 & 3.14 & 3.14 & 3.14 & 0.23 & 3.14 & 3.14 & 3.14 & 3.14 & 3.08 & 0.87 & 3.14 & 3.14 & 3.09 & 3.14 & 0.02 & 0.03 & 3.14 & 3.14 & 3.14 & 3.14 & 2.59 \\
CDS & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.02 & 0.00 & 0.00 & 0.00 & 0.00 & 0.02 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
\#GT & 1.00 & 0.00 & 0.00 & 61.00 & 242.00 & 66.00 & 340.00 & 0.00 & 0.00 & 399.00 & 0.00 & 0.00 & 0.00 & 0.00 & 149.00 & 2705.00 & 110.00 & 49.00 & 38.00 & 0.00 & 39.00 & 112.00 & 129.00 & 0.00 & 0.00 & 0.00 & 170.77 \\
\#Det & 123.00 & 0.00 & 0.00 & 1.00 & 252.00 & 328.00 & 0.00 & 0.00 & 0.00 & 215.00 & 0.00 & 0.00 & 0.00 & 0.00 & 24.00 & 5287.00 & 47.00 & 39.00 & 102.00 & 0.00 & 10.00 & 95.00 & 2.00 & 0.00 & 0.00 & 0.00 & 250.96 \\
\#TP & 0.00 & 0.00 & 0.00 & 0.00 & 6.25 & 0.50 & 0.00 & 0.00 & 0.00 & 11.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.50 & 405.75 & 0.00 & 0.25 & 2.00 & 0.00 & 1.25 & 5.25 & 0.00 & 0.00 & 0.00 & 0.00 & 16.64 \\
AR & 0.00 & 0.00 & 0.00 & 0.00 & 0.03 & 0.01 & 0.00 & 0.00 & 0.00 & 0.03 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.15 & 0.00 & 0.01 & 0.05 & 0.00 & 0.03 & 0.05 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 \\
\bottomrule
\end{tabular}
\end{table*}


==> tables/Tabulated_ImFSD_minpts=1_combined_50.tex <==
\begin{table*}
\footnotesize 
 \caption{Results from ImFSD minpts=1/combined 50.parquet}
\begin{tabular}{lrrrrrrrrrrrrrrrrrrrrrrrrrrr}
\toprule
 & \rot{Articulated Bus } & \rot{Bicycle } & \rot{Bicyclist } & \rot{Bollard } & \rot{Box Truck } & \rot{Bus } & \rot{Constr. Barrel } & \rot{Const. Cone } & \rot{Dog } & \rot{Large Vehicle } & \rot{Message Board Trailer } & \rot{M. Ped. Cross. Sign } & \rot{Motorcyle } & \rot{Motorcyclist } & \rot{Pedestrian } & \rot{Vehicle } & \rot{School Bus } & \rot{Sign } & \rot{Stop Sign } & \rot{Stroller } & \rot{Truck } & \rot{Truck Cab } & \rot{Trailer } & \rot{Wheelchair } & \rot{Wheeled Device } & \rot{Wheeled Rider } & \rot{Average Metrics } \\
\midrule
AP & 0.34 & 0.50 & 0.57 & 0.62 & 0.64 & 0.68 & 0.73 & 0.58 & 0.12 & 0.10 & 0.00 & 0.55 & 0.64 & 0.61 & 0.80 & 0.89 & 0.71 & 0.20 & 0.50 & 0.17 & 0.29 & 0.27 & 0.39 & 0.09 & 0.19 & 0.13 & 0.44 \\
ATE & 0.71 & 0.28 & 0.23 & 0.09 & 0.45 & 0.42 & 0.09 & 0.09 & 0.38 & 0.59 & 2.00 & 0.07 & 0.21 & 0.25 & 0.19 & 0.28 & 0.47 & 0.26 & 0.14 & 0.21 & 0.53 & 0.82 & 0.69 & 0.16 & 0.30 & 0.33 & 0.39 \\
ASE & 0.17 & 0.23 & 0.24 & 0.45 & 0.20 & 0.15 & 0.23 & 0.42 & 0.45 & 0.28 & 1.00 & 0.40 & 0.24 & 0.29 & 0.22 & 0.14 & 0.13 & 0.30 & 0.40 & 0.31 & 0.16 & 0.30 & 0.18 & 0.31 & 0.16 & 0.35 & 0.30 \\
AOE & 0.29 & 0.47 & 0.23 & 0.88 & 0.07 & 0.07 & 0.95 & 0.89 & 0.92 & 0.43 & 3.14 & 1.43 & 0.31 & 0.34 & 0.71 & 0.19 & 0.07 & 0.57 & 0.30 & 0.28 & 0.10 & 0.30 & 0.57 & 1.56 & 0.58 & 0.77 & 0.63 \\
CDS & 0.27 & 0.41 & 0.49 & 0.46 & 0.55 & 0.59 & 0.59 & 0.43 & 0.09 & 0.08 & 0.00 & 0.38 & 0.54 & 0.51 & 0.66 & 0.79 & 0.62 & 0.16 & 0.41 & 0.14 & 0.24 & 0.20 & 0.30 & 0.07 & 0.16 & 0.10 & 0.35 \\
\#GT & 755.00 & 13864.00 & 2480.00 & 55604.00 & 6543.00 & 5094.00 & 24962.00 & 24555.00 & 1375.00 & 5844.00 & 4.00 & 434.00 & 4592.00 & 1365.00 & 150560.00 & 375089.00 & 1095.00 & 7294.00 & 16362.00 & 635.00 & 4193.00 & 3517.00 & 5478.00 & 426.00 & 10074.00 & 1616.00 & 27838.85 \\
\#Det & 4729.00 & 54915.00 & 16655.00 & 116940.00 & 14242.00 & 11546.00 & 48984.00 & 64128.00 & 3090.00 & 22843.00 & 335.00 & 4761.00 & 22961.00 & 11080.00 & 260900.00 & 440502.00 & 3563.00 & 41704.00 & 56026.00 & 21575.00 & 14077.00 & 7190.00 & 15693.00 & 653.00 & 38267.00 & 14088.00 & 50440.27 \\
\#TP & 368.25 & 8891.75 & 1836.50 & 41112.25 & 4911.75 & 3881.75 & 19954.75 & 16880.75 & 478.75 & 2281.50 & 0.00 & 329.00 & 3508.25 & 1148.75 & 128759.50 & 342510.50 & 877.75 & 3408.00 & 10582.75 & 340.00 & 2382.25 & 1364.50 & 2774.75 & 124.00 & 3888.75 & 539.00 & 23197.53 \\
AR & 0.49 & 0.64 & 0.74 & 0.74 & 0.75 & 0.76 & 0.80 & 0.69 & 0.35 & 0.39 & 0.00 & 0.76 & 0.76 & 0.84 & 0.85 & 0.91 & 0.80 & 0.47 & 0.65 & 0.54 & 0.57 & 0.39 & 0.51 & 0.29 & 0.39 & 0.33 & 0.59 \\
\bottomrule
\end{tabular}
\end{table*}


==> tables/Tabulated_ImFSD_minpts=1_pts_0-250.tex <==
\begin{table*}
\footnotesize 
 \caption{Results from ImFSD minpts=1/pts 0-250.parquet}
\begin{tabular}{lrrrrrrrrrrrrrrrrrrrrrrrrrrr}
\toprule
 & \rot{Articulated Bus } & \rot{Bicycle } & \rot{Bicyclist } & \rot{Bollard } & \rot{Box Truck } & \rot{Bus } & \rot{Constr. Barrel } & \rot{Const. Cone } & \rot{Dog } & \rot{Large Vehicle } & \rot{Message Board Trailer } & \rot{M. Ped. Cross. Sign } & \rot{Motorcyle } & \rot{Motorcyclist } & \rot{Pedestrian } & \rot{Vehicle } & \rot{School Bus } & \rot{Sign } & \rot{Stop Sign } & \rot{Stroller } & \rot{Truck } & \rot{Truck Cab } & \rot{Trailer } & \rot{Wheelchair } & \rot{Wheeled Device } & \rot{Wheeled Rider } & \rot{Average Metrics } \\
\midrule
AP & 0.19 & 0.38 & 0.34 & 0.47 & 0.38 & 0.41 & 0.44 & 0.44 & 0.10 & 0.06 & 0.00 & 0.27 & 0.48 & 0.40 & 0.64 & 0.70 & 0.29 & 0.12 & 0.29 & 0.13 & 0.21 & 0.12 & 0.26 & 0.07 & 0.14 & 0.09 & 0.28 \\
ATE & 0.74 & 0.29 & 0.24 & 0.10 & 0.55 & 0.54 & 0.10 & 0.09 & 0.37 & 0.70 & 2.00 & 0.09 & 0.22 & 0.26 & 0.22 & 0.38 & 0.52 & 0.28 & 0.15 & 0.21 & 0.55 & 0.87 & 0.70 & 0.15 & 0.30 & 0.32 & 0.42 \\
ASE & 0.20 & 0.24 & 0.26 & 0.47 & 0.23 & 0.18 & 0.26 & 0.43 & 0.45 & 0.30 & 1.00 & 0.43 & 0.25 & 0.31 & 0.24 & 0.17 & 0.15 & 0.32 & 0.40 & 0.31 & 0.17 & 0.30 & 0.18 & 0.32 & 0.16 & 0.34 & 0.31 \\
AOE & 0.29 & 0.50 & 0.44 & 0.94 & 0.08 & 0.15 & 0.88 & 0.91 & 0.96 & 0.42 & 3.14 & 1.52 & 0.37 & 0.50 & 0.84 & 0.39 & 0.09 & 0.51 & 0.36 & 0.28 & 0.12 & 0.23 & 0.60 & 1.52 & 0.58 & 0.79 & 0.67 \\
CDS & 0.15 & 0.31 & 0.28 & 0.34 & 0.31 & 0.34 & 0.36 & 0.33 & 0.07 & 0.04 & 0.00 & 0.18 & 0.40 & 0.32 & 0.51 & 0.59 & 0.25 & 0.09 & 0.23 & 0.11 & 0.17 & 0.09 & 0.19 & 0.05 & 0.12 & 0.07 & 0.23 \\
\#GT & 1583.00 & 19389.00 & 5624.00 & 83827.00 & 15671.00 & 12908.00 & 49380.00 & 34103.00 & 1719.00 & 18004.00 & 68.00 & 1011.00 & 6334.00 & 2277.00 & 240461.00 & 746686.00 & 3127.00 & 13755.00 & 29729.00 & 822.00 & 8392.00 & 6825.00 & 10286.00 & 624.00 & 13824.00 & 2445.00 & 51110.54 \\
\#Det & 12058.00 & 67154.00 & 34245.00 & 170570.00 & 34324.00 & 30543.00 & 72113.00 & 77270.00 & 3191.00 & 49452.00 & 211.00 & 20249.00 & 34786.00 & 26641.00 & 461975.00 & 1020337.00 & 11384.00 & 71463.00 & 94791.00 & 26601.00 & 27539.00 & 14994.00 & 23902.00 & 586.00 & 41093.00 & 24616.00 & 94311.08 \\
\#TP & 505.75 & 9624.75 & 2727.25 & 49596.25 & 7418.00 & 6342.00 & 25119.25 & 18219.00 & 488.75 & 3642.25 & 0.00 & 434.50 & 3807.25 & 1438.00 & 169718.00 & 554725.75 & 1147.50 & 4138.75 & 12047.00 & 338.50 & 3535.75 & 1383.00 & 3405.25 & 121.25 & 3970.00 & 574.75 & 34018.02 \\
AR & 0.32 & 0.50 & 0.48 & 0.59 & 0.47 & 0.49 & 0.51 & 0.53 & 0.28 & 0.20 & 0.00 & 0.43 & 0.60 & 0.63 & 0.71 & 0.74 & 0.37 & 0.30 & 0.41 & 0.41 & 0.42 & 0.20 & 0.33 & 0.19 & 0.29 & 0.23 & 0.41 \\
\bottomrule
\end{tabular}
\end{table*}


==> tables/Tabulated_ImFSD_minpts=1_pts_100.tex <==
\begin{table*}
\footnotesize 
 \caption{Results from ImFSD minpts=1/pts 100.parquet}
\begin{tabular}{lrrrrrrrrrrrrrrrrrrrrrrrrrrr}
\toprule
 & \rot{Articulated Bus } & \rot{Bicycle } & \rot{Bicyclist } & \rot{Bollard } & \rot{Box Truck } & \rot{Bus } & \rot{Constr. Barrel } & \rot{Const. Cone } & \rot{Dog } & \rot{Large Vehicle } & \rot{Message Board Trailer } & \rot{M. Ped. Cross. Sign } & \rot{Motorcyle } & \rot{Motorcyclist } & \rot{Pedestrian } & \rot{Vehicle } & \rot{School Bus } & \rot{Sign } & \rot{Stop Sign } & \rot{Stroller } & \rot{Truck } & \rot{Truck Cab } & \rot{Trailer } & \rot{Wheelchair } & \rot{Wheeled Device } & \rot{Wheeled Rider } & \rot{Average Metrics } \\
\midrule
AP & 0.06 & 0.09 & 0.20 & 0.16 & 0.24 & 0.31 & 0.19 & 0.07 & 0.03 & 0.05 & 0.00 & 0.11 & 0.10 & 0.08 & 0.41 & 0.60 & 0.09 & 0.04 & 0.04 & 0.00 & 0.18 & 0.10 & 0.12 & 0.01 & 0.00 & 0.01 & 0.13 \\
ATE & 0.96 & 0.40 & 0.28 & 0.18 & 0.66 & 0.69 & 0.14 & 0.13 & 0.26 & 0.74 & 2.00 & 0.14 & 0.36 & 0.33 & 0.30 & 0.49 & 0.64 & 0.34 & 0.24 & 0.54 & 0.60 & 0.83 & 0.80 & 0.13 & 0.44 & 0.34 & 0.50 \\
ASE & 0.33 & 0.34 & 0.28 & 0.55 & 0.27 & 0.21 & 0.34 & 0.54 & 0.45 & 0.32 & 1.00 & 0.50 & 0.33 & 0.37 & 0.31 & 0.20 & 0.19 & 0.35 & 0.43 & 0.60 & 0.20 & 0.30 & 0.23 & 0.53 & 0.30 & 0.34 & 0.38 \\
AOE & 0.61 & 0.86 & 0.79 & 1.20 & 0.11 & 0.25 & 0.58 & 1.03 & 1.59 & 0.53 & 3.14 & 1.61 & 0.91 & 1.06 & 1.22 & 0.63 & 0.13 & 0.41 & 0.77 & 1.13 & 0.20 & 0.14 & 0.83 & 1.55 & 0.91 & 0.85 & 0.89 \\
CDS & 0.04 & 0.07 & 0.15 & 0.11 & 0.19 & 0.24 & 0.15 & 0.05 & 0.02 & 0.04 & 0.00 & 0.07 & 0.07 & 0.06 & 0.29 & 0.47 & 0.08 & 0.03 & 0.03 & 0.00 & 0.15 & 0.07 & 0.09 & 0.01 & 0.00 & 0.01 & 0.10 \\
\#GT & 558.00 & 4131.00 & 2018.00 & 23300.00 & 5214.00 & 3772.00 & 15093.00 & 7296.00 & 341.00 & 5079.00 & 64.00 & 448.00 & 1219.00 & 547.00 & 66309.00 & 245887.00 & 1061.00 & 4078.00 & 9056.00 & 175.00 & 2764.00 & 1831.00 & 2790.00 & 150.00 & 3051.00 & 666.00 & 15649.92 \\
\#Det & 5984.00 & 12398.00 & 16706.00 & 51730.00 & 12741.00 & 11347.00 & 23033.00 & 15528.00 & 187.00 & 18486.00 & 1.00 & 7081.00 & 11887.00 & 14462.00 & 179008.00 & 379771.00 & 4840.00 & 20910.00 & 26493.00 & 5065.00 & 11024.00 & 5695.00 & 8562.00 & 25.00 & 3717.00 & 12480.00 & 33044.65 \\
\#TP & 112.75 & 900.50 & 898.50 & 8522.00 & 2008.75 & 1706.50 & 4932.50 & 1614.50 & 23.75 & 1107.00 & 0.00 & 101.00 & 409.50 & 312.75 & 38024.75 & 165199.25 & 254.00 & 929.75 & 1589.00 & 2.75 & 1176.25 & 374.50 & 599.50 & 3.00 & 121.75 & 82.50 & 8884.89 \\
AR & 0.20 & 0.22 & 0.45 & 0.37 & 0.39 & 0.45 & 0.33 & 0.22 & 0.07 & 0.22 & 0.00 & 0.23 & 0.34 & 0.57 & 0.57 & 0.67 & 0.24 & 0.23 & 0.17 & 0.02 & 0.43 & 0.20 & 0.21 & 0.02 & 0.04 & 0.12 & 0.27 \\
\bottomrule
\end{tabular}
\end{table*}


==> tables/Tabulated_ImFSD_minpts=1_pts_150.tex <==
\begin{table*}
\footnotesize 
 \caption{Results from ImFSD minpts=1/pts 150.parquet}
\begin{tabular}{lrrrrrrrrrrrrrrrrrrrrrrrrrrr}
\toprule
 & \rot{Articulated Bus } & \rot{Bicycle } & \rot{Bicyclist } & \rot{Bollard } & \rot{Box Truck } & \rot{Bus } & \rot{Constr. Barrel } & \rot{Const. Cone } & \rot{Dog } & \rot{Large Vehicle } & \rot{Message Board Trailer } & \rot{M. Ped. Cross. Sign } & \rot{Motorcyle } & \rot{Motorcyclist } & \rot{Pedestrian } & \rot{Vehicle } & \rot{School Bus } & \rot{Sign } & \rot{Stop Sign } & \rot{Stroller } & \rot{Truck } & \rot{Truck Cab } & \rot{Trailer } & \rot{Wheelchair } & \rot{Wheeled Device } & \rot{Wheeled Rider } & \rot{Average Metrics } \\
\midrule
AP & 0.04 & 0.00 & 0.01 & 0.02 & 0.08 & 0.15 & 0.01 & 0.00 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.11 & 0.27 & 0.00 & 0.00 & 0.00 & 0.00 & 0.05 & 0.03 & 0.04 & 0.00 & 0.01 & 0.00 & 0.03 \\
ATE & 0.52 & 0.52 & 0.41 & 0.27 & 0.91 & 0.80 & 0.20 & 0.18 & 2.00 & 0.95 & 2.00 & 0.21 & 0.53 & 0.37 & 0.41 & 0.66 & 1.06 & 0.43 & 0.38 & 2.00 & 0.71 & 0.98 & 0.72 & 2.00 & 0.47 & 0.29 & 0.77 \\
ASE & 0.14 & 0.37 & 0.33 & 0.56 & 0.33 & 0.22 & 0.57 & 0.53 & 1.00 & 0.37 & 1.00 & 0.64 & 0.43 & 0.48 & 0.38 & 0.25 & 0.29 & 0.40 & 0.41 & 1.00 & 0.23 & 0.26 & 0.20 & 1.00 & 0.29 & 0.43 & 0.47 \\
AOE & 0.12 & 1.43 & 1.64 & 1.33 & 0.19 & 0.29 & 1.14 & 1.54 & 3.14 & 0.39 & 3.14 & 2.88 & 2.09 & 2.68 & 1.39 & 0.90 & 0.34 & 0.11 & 0.99 & 3.14 & 0.19 & 0.23 & 1.20 & 3.14 & 0.14 & 3.02 & 1.42 \\
CDS & 0.04 & 0.00 & 0.01 & 0.01 & 0.06 & 0.12 & 0.01 & 0.00 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.07 & 0.19 & 0.00 & 0.00 & 0.00 & 0.00 & 0.04 & 0.02 & 0.03 & 0.00 & 0.00 & 0.00 & 0.02 \\
\#GT & 205.00 & 1251.00 & 934.00 & 3952.00 & 2316.00 & 2500.00 & 6630.00 & 2171.00 & 3.00 & 4045.00 & 0.00 & 114.00 & 498.00 & 347.00 & 20343.00 & 97700.00 & 574.00 & 1664.00 & 3259.00 & 12.00 & 1100.00 & 899.00 & 1223.00 & 48.00 & 669.00 & 154.00 & 5869.65 \\
\#Det & 1434.00 & 918.00 & 3369.00 & 3101.00 & 7262.00 & 6159.00 & 2985.00 & 103.00 & 0.00 & 8962.00 & 0.00 & 7935.00 & 1347.00 & 2301.00 & 36570.00 & 181237.00 & 2918.00 & 7868.00 & 11318.00 & 788.00 & 5360.00 & 2692.00 & 2245.00 & 0.00 & 77.00 & 822.00 & 11452.73 \\
\#TP & 41.00 & 45.75 & 86.25 & 291.00 & 527.50 & 703.25 & 380.75 & 6.00 & 0.00 & 492.00 & 0.00 & 20.50 & 19.50 & 23.75 & 5143.75 & 39474.50 & 39.00 & 162.00 & 247.75 & 0.00 & 226.75 & 83.50 & 109.00 & 0.00 & 4.50 & 1.00 & 1851.12 \\
AR & 0.20 & 0.04 & 0.09 & 0.07 & 0.23 & 0.28 & 0.06 & 0.00 & 0.00 & 0.12 & 0.00 & 0.18 & 0.04 & 0.07 & 0.25 & 0.40 & 0.07 & 0.10 & 0.08 & 0.00 & 0.21 & 0.09 & 0.09 & 0.00 & 0.01 & 0.01 & 0.10 \\
\bottomrule
\end{tabular}
\end{table*}


==> tables/Tabulated_ImFSD_minpts=1_pts_200.tex <==
\begin{table*}
\footnotesize 
 \caption{Results from ImFSD minpts=1/pts 200.parquet}
\begin{tabular}{lrrrrrrrrrrrrrrrrrrrrrrrrrrr}
\toprule
 & \rot{Articulated Bus } & \rot{Bicycle } & \rot{Bicyclist } & \rot{Bollard } & \rot{Box Truck } & \rot{Bus } & \rot{Constr. Barrel } & \rot{Const. Cone } & \rot{Dog } & \rot{Large Vehicle } & \rot{Message Board Trailer } & \rot{M. Ped. Cross. Sign } & \rot{Motorcyle } & \rot{Motorcyclist } & \rot{Pedestrian } & \rot{Vehicle } & \rot{School Bus } & \rot{Sign } & \rot{Stop Sign } & \rot{Stroller } & \rot{Truck } & \rot{Truck Cab } & \rot{Trailer } & \rot{Wheelchair } & \rot{Wheeled Device } & \rot{Wheeled Rider } & \rot{Average Metrics } \\
\midrule
AP & 0.00 & 0.00 & 0.00 & 0.00 & 0.03 & 0.01 & 0.00 & 0.00 & 0.00 & 0.02 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.12 & 0.00 & 0.01 & 0.00 & 0.00 & 0.01 & 0.04 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 \\
ATE & 0.71 & 2.00 & 0.69 & 2.00 & 1.16 & 0.95 & 2.00 & 2.00 & 2.00 & 1.15 & 2.00 & 2.00 & 2.00 & 2.00 & 0.50 & 0.72 & 1.08 & 0.60 & 0.41 & 2.00 & 0.59 & 1.13 & 0.76 & 2.00 & 2.00 & 2.00 & 1.40 \\
ASE & 0.22 & 1.00 & 0.28 & 1.00 & 0.41 & 0.31 & 1.00 & 1.00 & 1.00 & 0.38 & 1.00 & 1.00 & 1.00 & 1.00 & 0.43 & 0.28 & 0.25 & 0.47 & 0.34 & 1.00 & 0.28 & 0.24 & 0.36 & 1.00 & 1.00 & 1.00 & 0.66 \\
AOE & 0.32 & 3.14 & 0.04 & 3.14 & 0.29 & 0.51 & 3.14 & 3.14 & 3.14 & 0.25 & 3.14 & 3.14 & 3.14 & 3.14 & 1.55 & 0.94 & 0.05 & 0.13 & 0.08 & 3.14 & 0.41 & 0.17 & 0.25 & 3.14 & 3.14 & 3.14 & 1.76 \\
CDS & 0.00 & 0.00 & 0.00 & 0.00 & 0.02 & 0.01 & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.08 & 0.00 & 0.01 & 0.00 & 0.00 & 0.01 & 0.03 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 \\
\#GT & 64.00 & 143.00 & 192.00 & 910.00 & 1356.00 & 1476.00 & 2355.00 & 81.00 & 0.00 & 2637.00 & 0.00 & 15.00 & 25.00 & 18.00 & 3100.00 & 25305.00 & 287.00 & 670.00 & 1014.00 & 0.00 & 296.00 & 466.00 & 666.00 & 0.00 & 30.00 & 9.00 & 1581.35 \\
\#Det & 839.00 & 22.00 & 105.00 & 5.00 & 2904.00 & 3199.00 & 4.00 & 0.00 & 0.00 & 3545.00 & 0.00 & 941.00 & 8.00 & 12.00 & 910.00 & 39302.00 & 968.00 & 1903.00 & 1628.00 & 0.00 & 760.00 & 1411.00 & 296.00 & 0.00 & 2.00 & 0.00 & 2260.15 \\
\#TP & 9.00 & 0.00 & 1.75 & 0.00 & 170.50 & 112.25 & 0.25 & 0.00 & 0.00 & 252.00 & 0.00 & 0.00 & 0.00 & 0.00 & 100.25 & 6486.75 & 8.25 & 25.75 & 35.00 & 0.00 & 20.00 & 41.25 & 13.25 & 0.00 & 0.00 & 0.00 & 279.86 \\
AR & 0.14 & 0.00 & 0.01 & 0.00 & 0.13 & 0.08 & 0.00 & 0.00 & 0.00 & 0.10 & 0.00 & 0.00 & 0.00 & 0.00 & 0.03 & 0.26 & 0.03 & 0.04 & 0.04 & 0.00 & 0.07 & 0.09 & 0.02 & 0.00 & 0.00 & 0.00 & 0.04 \\
\bottomrule
\end{tabular}
\end{table*}


==> tables/Tabulated_ImFSD_minpts=1_pts_50.tex <==
\begin{table*}
\footnotesize 
 \caption{Results from ImFSD minpts=1/pts 50.parquet}
\begin{tabular}{lrrrrrrrrrrrrrrrrrrrrrrrrrrr}
\toprule
 & \rot{Articulated Bus } & \rot{Bicycle } & \rot{Bicyclist } & \rot{Bollard } & \rot{Box Truck } & \rot{Bus } & \rot{Constr. Barrel } & \rot{Const. Cone } & \rot{Dog } & \rot{Large Vehicle } & \rot{Message Board Trailer } & \rot{M. Ped. Cross. Sign } & \rot{Motorcyle } & \rot{Motorcyclist } & \rot{Pedestrian } & \rot{Vehicle } & \rot{School Bus } & \rot{Sign } & \rot{Stop Sign } & \rot{Stroller } & \rot{Truck } & \rot{Truck Cab } & \rot{Trailer } & \rot{Wheelchair } & \rot{Wheeled Device } & \rot{Wheeled Rider } & \rot{Average Metrics } \\
\midrule
AP & 0.34 & 0.50 & 0.60 & 0.62 & 0.66 & 0.69 & 0.74 & 0.58 & 0.12 & 0.12 & 0.00 & 0.54 & 0.64 & 0.63 & 0.81 & 0.89 & 0.72 & 0.20 & 0.50 & 0.17 & 0.29 & 0.17 & 0.41 & 0.10 & 0.19 & 0.14 & 0.44 \\
ATE & 0.68 & 0.28 & 0.22 & 0.09 & 0.44 & 0.41 & 0.09 & 0.09 & 0.38 & 0.57 & 2.00 & 0.06 & 0.21 & 0.25 & 0.19 & 0.28 & 0.45 & 0.26 & 0.14 & 0.21 & 0.53 & 0.86 & 0.68 & 0.15 & 0.30 & 0.33 & 0.39 \\
ASE & 0.17 & 0.23 & 0.24 & 0.45 & 0.19 & 0.15 & 0.23 & 0.42 & 0.45 & 0.27 & 1.00 & 0.40 & 0.24 & 0.29 & 0.22 & 0.14 & 0.13 & 0.30 & 0.40 & 0.31 & 0.16 & 0.31 & 0.17 & 0.31 & 0.16 & 0.34 & 0.29 \\
AOE & 0.20 & 0.47 & 0.23 & 0.88 & 0.06 & 0.06 & 0.95 & 0.89 & 0.94 & 0.42 & 3.14 & 1.41 & 0.31 & 0.33 & 0.71 & 0.19 & 0.06 & 0.56 & 0.30 & 0.28 & 0.08 & 0.28 & 0.54 & 1.52 & 0.57 & 0.79 & 0.62 \\
CDS & 0.27 & 0.41 & 0.51 & 0.46 & 0.56 & 0.60 & 0.60 & 0.43 & 0.08 & 0.09 & 0.00 & 0.38 & 0.54 & 0.53 & 0.66 & 0.79 & 0.63 & 0.16 & 0.41 & 0.14 & 0.25 & 0.13 & 0.31 & 0.07 & 0.16 & 0.10 & 0.36 \\
\#GT & 755.00 & 13864.00 & 2480.00 & 55604.00 & 6543.00 & 5094.00 & 24962.00 & 24555.00 & 1375.00 & 5844.00 & 4.00 & 434.00 & 4592.00 & 1365.00 & 150560.00 & 375089.00 & 1095.00 & 7294.00 & 16362.00 & 635.00 & 4193.00 & 3517.00 & 5478.00 & 426.00 & 10074.00 & 1616.00 & 27838.85 \\
\#Det & 3767.00 & 53816.00 & 14065.00 & 116312.00 & 11254.00 & 9684.00 & 46091.00 & 61639.00 & 3004.00 & 18335.00 & 210.00 & 4289.00 & 21544.00 & 9866.00 & 250689.00 & 432356.00 & 2614.00 & 40760.00 & 55350.00 & 20748.00 & 10387.00 & 5115.00 & 12799.00 & 561.00 & 37297.00 & 11314.00 & 48225.61 \\
\#TP & 355.00 & 8838.50 & 1826.25 & 41094.25 & 4905.50 & 3860.00 & 19859.00 & 16779.00 & 467.00 & 2201.25 & 0.00 & 319.25 & 3464.25 & 1147.00 & 128719.25 & 342270.75 & 865.50 & 3391.25 & 10580.25 & 340.75 & 2266.75 & 900.50 & 2738.00 & 118.25 & 3860.75 & 535.75 & 23142.46 \\
AR & 0.47 & 0.64 & 0.74 & 0.74 & 0.75 & 0.76 & 0.80 & 0.68 & 0.34 & 0.38 & 0.00 & 0.74 & 0.75 & 0.84 & 0.85 & 0.91 & 0.79 & 0.47 & 0.65 & 0.54 & 0.54 & 0.26 & 0.50 & 0.28 & 0.38 & 0.33 & 0.58 \\
\bottomrule
\end{tabular}
\end{table*}

